Meterstick: Benchmarking Performance Variability in Cloud and Self-hosted Minecraft-like Games Extended Technical Report

Due to increasing popularity and strict performance requirements, online games have become a workload of interest for the performance engineering community. One of the most popular types of online games is the Minecraft-like Game (MLG), in which players can terraform the environment. The most popular MLG, Minecraft, provides not only entertainment, but also educational support and social interaction, to over 130 million people world-wide. MLGs currently support their many players by replicating isolated instances that support each only up to a few hundred players under favorable conditions. In practice, as we show here, the real upper limit of supported players can be much lower. In this work, we posit that performance variability is a key cause for the lack of scalability in MLGs. We propose a novel operational model for MLGs and use it to design the first benchmark that focuses on MLG performance variability, defining specialized workloads, metrics, and processes. We conduct real-world benchmarking of MLGs and find environment-based workloads and cloud deployment to be significant sources of performance variability: peak-latency degrades sharply to 20.7 times the arithmetic mean, and exceeds by a factor of 7.4 the performance requirements. We derive actionable insights for game-developers, game-operators, and other stakeholders to tame performance variability.

==> TECHNICAL REPORT ICPE2023 Meterstick NEW/content/00-abstract.tex <==
Due to increasing popularity and strict performance requirements, online games have become a
% cloud-based and self-hosted
workload of interest for the performance engineering community.
One of the most popular types of online games is the \mve, in which players can terraform the environment. The most popular \mve, Minecraft, provides not only entertainment, but also educational support and social interaction, to over 130\,million people world-wide.
\mves currently support their many players by replicating isolated instances that support each only up to a few hundred players under favorable conditions.
In practice, as we show here, the real upper limit of supported players can be much lower.
In this work, we posit that performance variability is a key cause for the lack of scalability in \mves.
% investigate experimentally causes of performance variability, and derive actionable insights.
We propose a novel operational model for \mves
% which extends the state-of-the-art with essential aspects, e.g., through the consideration of \envworkloads,
% which are sizable workload components that do not depend on player input (once set in action).
% Starting from this model,
and use it to design the first benchmark that focuses on \mve performance variability, defining specialized workloads, metrics, and processes.
We conduct real-world benchmarking of \mves
% , both cloud-based and self-hosted.
and find \envworkloads and cloud deployment to be significant sources of performance variability: peak-latency degrades sharply to 20.7~times the arithmetic mean, and exceeds by a factor of 7.4~the performance requirements.
We derive actionable insights for game-developers, game-operators, and other stakeholders to tame performance variability.


% OLDER VERSIONS
% Games provide entertainment, educational support, and social interaction to 3~billion gamers around the world,
% and have become the largest entertainment industry world-wide.
% One of the most popular types of game is the \mve,
% in which players can terraform the environment. %have fine-grained control over the environment and can modify it at will.
% The canonical example of an \mve is Minecraft, which is the best-selling game of all time, and has more active users than MacOS.
% However, \mves face an important scalability challenge, only supporting their large player numbers by replicating isolated instances, preventing players from playing together.
% While previous work has shown that these games can support a few hundred players under favorable conditions,
% the real number of supported players can be much lower due to significant performance variability.
% In this work, we propose an operational model for \mves,
% and use this model to design the first benchmark that evaluates \mve performance variability. %, using our novel \emph{jitter} metric.
% Using our benchmark, we find \emph{\envworkloads} and cloud deployment to be significant sources of performance variability, with peak-latency reaching values 20.7~times the arithmetic mean and exceeding by a factor of 7.4~the worst-case acceptable limits.
% Based on our findings, we present actionable insights for stakeholders to limit the impact of this performance variability.
% %We find that both the varying workload and deployment environment have significant impact on the game's performance and performance variability,
% %and recommended hardware is insufficient.

% % Minecraft-like games represent an increasingly common use case for Infrastructure as a Service (IaaS) providers [REF 3x]. \todo[inline]{find refs}These games are characterized by the operation of large-scale, real-time, dynamic, multi-user modifiable virtual environments (MVEs) with corresponding strict quality of service requirements. Unlike comparable real-time systems such as video conferencing, video game architectures operate intensive dynamic simulations alongside maintaining state consistency for users, creating complex performance behaviors that cannot easily be predicted. Although Minecraft-like games are both prevalent and operationally complex, the real-world performance characteristics of Minecraft-like games, and video game systems in general, remain under-studied. As Minecraft-like games are increasingly more frequently operated in IaaS environments, understanding their performance profile is key to developing resource allocation and scheduling 
% % techniques that minimize resource usage while still meeting quality of service requirements. To inform such research, we propose a fine-grained operational model for Minecraft-like games. Ours is the first such model to consider player-agnostic 
% % workloads, which are parts of the general Minecraft-like model that operate and update without further input from the player, creating (as we show) significant workload but also giving room for optimization that is not hampered by the volatility of player inputs. Then, we use this model to design a benchmark for Minecraft-like games deployed in real-world cloud environments, using as input realistic workloads of the kind defined by our model, and producing a variety of standard metrics as well as a new statistical analysis unique to Minecraft-like games that produced a single-figure performance score. Finally, we conduct extensive real-world experiments on three common implementations of Minecraft-like games and the two most popular IaaS providers and analyze the results. From these experiments, our analysis indicates that Minecraft-like games in commercial cloud environments exhibit high degrees of performance variability (from X[\%] to Y[\%], with a median of Z[\%]) and that workload characteristics strongly influence the performance variability patterns [DETAIL FOR THIS CONTRIBUTION]. Our results indicate there is good potential for more advanced resource allocation techniques that account for workload-induced performance variability in commercial cloud environments.


==> TECHNICAL REPORT ICPE2023 Meterstick NEW/content/1_introduction.tex <==

\section{Introduction}
\label{sec:intro}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/rtt_box_simple.pdf}
    \vspace*{-0.65cm}
    %\caption{Response time of Minecraft when running in the AWS cloud.}
    \caption{Minecraft response time in the AWS cloud.}
    \label{fig:preview_result}
    \vspace*{-0.5cm}
\end{figure}

% First paragraph
The gaming industry is the world's largest entertainment industry~\cite{gamingbiggestindustry}---world-wide, games engage over 3~billion players and yield over \$170~billion in revenue~\cite{newzoo2021}.
% The revenue of the global video game industry grew throughout 2020 to 180 billion USD, a value greater than the global movie and North American sports combined~\cite{marketwatch2020}.
In this work, we focus on \emph{Minecraft-like Games (\mves)}, an emergent and highly popular type of game where users can change almost every part of the environment.
The canonical example of an \mve is Minecraft, which is already the best-selling game of all time~\cite{Madan2019May}.
% Minecraft remains highly popular with over 131 million active players per month~\cite{2windows2020}\footnote{Factually, Minecraft has more players than MacOS has users~\cite{Warren2017Apr}.}.
%\mves distinguish themselves from other games through their use of computationally complex environments, and giving players fine-grained control over these environments.
All \mves, including Minecraft, present an important challenge to the performance engineering community: although their user-bases can exceed 100 million active users per month\remove{\footnote{Minecraft has over 130\,million active users/month~\cite{2windows2020}, more than, e.g., MacOS~\cite{Warren2017Apr}.}}, their \textit{scalability} is limited to only 200-300 players even under very favorable conditions~\cite{yardstick}. (\mves support high concurrency by creating separate replicas of their virtual worlds, essentially sharding state and not allowing cross-instance interaction.)
\textit{What limits \mve scalability?} %is the key question we investigate in this work. 
In this work,
we posit performance variability is a key limit to \mve scalability,
and design and use an \mve benchmark focusing on this concept.

% Even under favorable conditions, previous work has shown that \mves can scale only up to 200-300 players~\cite{yardstick}; to 
% important scalability challenge for the performance 
% But although \mves are highly popular, their scalability is limited, effectively preventing players from playing together.
% Although previous work has shown that \mves scale to 200-300 players under favorable conditions~\cite{yardstick},
% their scalability in practice can be much lower due to significant performance variability.
% % Although these features appeal to a large audience,
% % they can significantly impact the game's performance variability and performance overall.
% % \todoall{This is indeed a problem for Minecraft, but not the problem we are addressing. Change the storyline to address only ONE problem (one "However" or "Although"), ours.}
% % \todoall{To address this problem, we need to understand more about this performance variability (how it happens, why it happens, what we can do about it)}
% In this work, we propose an operational model for \mves, and use it to design \toolname, a benchmark that quantifies performance variability in \mves.
% We use \toolname to analyze \mve behavior under realistic workloads and deployment environments. 

% The revenue of the global video game industry grew throughout 2020 to 180 billion USD, a value greater than the global movie and North American sports combined~\cite{marketwatch2020}. Video gaming has become an integral part of every day life, as well as a communicative tool with vast international influence. However, video games as a online service represent a largely under-studied optimization challenge. The player experience of online games is dependent on achieving minimal latency for real-time networking. Technological advances in consumer-grade hardware have delayed this problem for traditional game styles by allowing higher network throughput, as well as facilitating load distribution through alternative service architectures such as peer-to-peer. However, there is an important class of video games that remains a performance challenge, that of \emph{Minecraft-like games}.

% Context - What is an MVE?
\mves represent an important and unique class of online multiplayer games.
Most importantly, \mves allow players to create, modify, and remove in-game objects (e.g., player apparel) and geographical features (e.g., terrain)~\cite{DBLP:conf/hotcloud/DonkervlietTI20}.
% Players can and do significantly change the virtual environment by 
% building (e.g., creating cities) and terraforming (e.g., moving mountains). 
Moreover, some game objects and features are self-acting, that is, they act even when no player input is applied to them. Players can use them to create dynamic elements, by ``programming'' the environment with combinations of self-acting parts.

% % Context - MVEs in society
% \mves are also an important class of software artifacts to study and improve:
% although Minecraft is currently the best known example of an \mve,
% thousands of commercial \mves exist and a rich modding community of tens of thousands of developers has emerged around \mves.
% %which give players the ability to modify the environment and create dynamic elements.
% % \remove{Beyond gaming, \mves also act as platforms for many societally relevant activities, e.g., as safe-havens for press fighting against real-world censorship~\cite{uncensored}, as collaborative urban-design tools~\cite{blockbyblock}, as visualization tools for metabolic pathways~\cite{metabolics}, and as safe-spaces for autistic people~\cite{autcraft, autexpression}.}


% Minecraft-like games are characterized by the operation of \emph{modifiable virtual environments (MVEs)}, which are simulated in real time and allow nearly unbounded player modifications. The most popular of these games, Minecraft itself, is one of the best selling game of all time~\cite{1windows2020} and reports over 131 million players per month~\cite{2windows2020}. Minecraft has not only functioned as an entertainment medium, but as a platform for social movements with a broad spectrum of causes, from facilitating an in-game haven for press freedom to fight against real world censorship~\cite{uncensored}, seeking to build the entirety of Earth~\cite{buildearth}, creating visualization tools for metabolic pathways~\cite{metabolics}, and creating safe spaces for autistic players~\cite{autcraft, autexpression}.

% Minecraft's popularity has both inspired and popularized a variety of Minecraft-like games with similar features. Notable examples are No Man's Sky~\cite{nomanssky}, Astroneer~\cite{astroneer}, Terraria~\cite{terraria}, and Space Engineers~\cite{spaceengineer}.

% Problem statement
\textit{Performance variability} prevents \mve service providers from giving strict \qos guarantees,
and simultaneously incentivizes overprovisioning of resources and limiting
the number of players that can interact together.
For example, Minecraft Realms, a Minecraft \textit{cloud-based service} offered by Microsoft, limits the %maximum number of players in a single instance to only ten (10)\textbf{!}
number of players per game-instance to at most 10~(ten)\textbf{!}
In contrast, Hypixel, at 216,762 online players~\cite{minetrack} the most populated Minecraft server, achieves high player-count by stitching together thousands of (independent) \mve instances using specialized tools, but players in different instances cannot interact.

In this work, \emph{we show for the first time empirical evidence that current \mves experience significant performance variability}.
%, a performance phenomenon that is currently not well understood.
Figure~\ref{fig:preview_result} depicts an exemplary result---% of performance variability in \mves---
even with a single connected player, the response time varies from good~(below 60\,ms) to \textit{unplayable}~(above 118\,ms). We discuss this and similar real-world experiments in \Cref{sec:mf1}.

% Performance variability prevents \mve service providers from giving strict \qos guarantees,
% and simultaneously incentivizes overprovisioning of resources and limiting
% the number of players that can interact together.
% For example, Minecraft Realms, a Minecraft \textit{cloud-based service} offered by Microsoft, limits the %maximum number of players in a single instance to only ten (10)\textbf{!}
% number of players per game-instance to at most 10~(ten)\textbf{!}
% % The operators of Minecraft-like game servers have the choice to host using commercially available cloud computing providers. Mojang itself, the company that develops Minecraft, chose to host Minecraft Realms, their server hosting service, on Amazon Web Services~\cite{RealmsAWS}\footnote{In early 2021 Mojang migrated Realms entirely to Microsoft Azure.} rather than their own hardware.
% % \todo[inline]{Find better explanation of cloud hosting popularity}
% % From a consumer, rather than corporate, perspective, the option of cloud deployment instead of self-hosting would be taken to gain access to more computational power without a large budget, or to have a stable network configuration that allows players to connect without going through a host's private network. While there is no available data on the amount of server operators choosing to host on cloud environments, the popularity of doing so can be seen in the growing plethora of cloud computing services specifically marketed for Minecraft or other Minecraft-like games. An incomplete survey of these services is available in Appendix~\ref{sec:appendix_a}.
% %
% \add{In contrast, Hypixel, the largest Minecraft server with a record of 216,762 online players~\cite{minetrack}, stitches together thousands of \mve instances using specialized tools to achieve high player-count, but even then players in different instances cannot interact.}
% %\info{R3C1}


Furthermore, \textit{ours is the first study to systematically analyze the effects of performance variability on the operation of \mves.} By designing and using for this purpose a novel benchmark, we provide an important complement to an emerging body of knowledge.
Game researchers and engineers are already aware of the impact of several types of performance variability.
Performance variability in networks causes players to stop playing sooner~\cite{DBLP:journals/cacm/ChenHL06},
and there are widespread techniques in industry to prevent variability in frame rates~\cite{UnityMan69:online,DynamicR99:online}.
However, the effect of performance variability on the interactive simulation of virtual worlds, and in particular on \mves, is much less understood.
% poorly
% understood, while this can cause large spikes in the game's response time.
% \info{R1C2}

% Related work
Prior work in understanding the performance of \mves~\cite{yardstick,DBLP:journals/corr/abs-1907-13440} and on improving their scalability~\cite{DBLP:conf/netgames/DiaconuKV13,DBLP:conf/netgames/EngelbrechtS13,DBLP:conf/icdcs/DonkervlietCI21} forms a valuable contribution to the field, but does not currently consider explicitly performance variability.
Addressing this important gap, we make a four-fold contribution:

\begin{myitemize}[label=\textbf{C\arabic*}]
    \item\label{contrib:model} We propose an operational model of \mves.
    Ours is the first to consider \mve-specific workloads (\Cref{sec:mve-workload-model}).
    % These workload are caused by simulating the virtual environment, are largely independent from the number of online players, and cause significant performance variability.
    Because \mves allow players to program the virtual environment and terraform the terrain, they support new types of workload not available in most traditional online games.
    %This work is the first to study this type of workload, and its impact on performance variability.
    % \item We propose a fine-grained operational model for Minecraft-like games. Ours is the first such model to consider player-agnostic workloads, which are parts of the general Minecraft-like model that operate and update without further input from the player, creating (as we show) significant workload but also giving room for optimization that is not hampered by the volatility of player inputs.

    \item\label{contrib:design} We design \toolname, a benchmark that quantifies performance variability in \mves (\Cref{sec:design}).
    To this end, we propose a novel performance variability metric, and define a benchmarking approach to produce it experimentally.
    Our benchmark
    %includes representative
    % % \envworkloads
    % \mve-specific workloads
    % and
    % % \mves deployed in commercial cloud environments.
    supports common deployment-environments for \mves offered as a service, in particular, both cloud-based and self-hosted.
    Our benchmark is the first to quantify performance variability in \mves.

    \item\label{contrib:experiments} We conduct real-world experiments using \toolname~(\Cref{sec:experiments}) and, after analyzing the results, propose actionable insights~(\Cref{sec:actionable_insights}). We evaluate the performance variability of three popular \mves, running on two popular commercial cloud providers and one local compute-cluster.
    % We investigate how their performance variability is affected by \mve-specific workloads and their deployment-environment, and derive actionable insights.
    % We conduct experiments on two popular commercial cloud providers and one local compute cluster.

    % Our experiments show that performance variability caused by \envworkloads in real-world commercial cloud platforms can cause \mves to fail to maintain quality of service with only a single player in the game, significantly lowering the maximum number of supported players reported in earlier work~\cite{yardstick}.

    \item\label{contrib:FAIR} Following open-science and reproducibility principles, we publish {Findable, Accessible, Interoperable, and Reusable (FAIR~\cite{data:FAIR16})} data, available on Zenodo~\cite{meterstick:data:orig}, and Free-access Open-Source Software (FOSS) artifacts, available on GitHub~\cite{meterstick:git}. %~(anonymized).
    % \end{enumerate}
\end{myitemize}


==> TECHNICAL REPORT ICPE2023 Meterstick NEW/content/2_operational_model.tex <==

\section{Operational Model of Minecraft-like Games}
\label{sec:mve-workload-model}
\label{sec:model}

For contribution~\ref{contrib:model}, first, we summarize a state-of-the-art % fine-grained 
operational model and a reference architecture for \mves~(\Cref{sec:model:mve-archi}).
%, where the explicit network protocol and state model greatly extend the state-of-the-art; \Cref{sec:model:mve-archi} defines our reference architecture for \mves.
Second, we define \mve-specific \emph{\envworkloads} that are caused by terrain and entity simulation; \Cref{sec:model:workloads} defines the resulting \mve workload model.
Third, %and finally, 
we model the operational elements of these workloads~(\Cref{sec:model:operational}).

% and define \emph{\envworkloads} as \mve-specific workloads, caused by terrain and entity simulation.
% First, we describe a reference architecture for \mves~(\Cref{sec:model:mve-archi}).
% Second, we present a model for \mve workloads, which includes \envworkloads~(\Cref{sec:model:workloads}).
% Third, and finally, we model the operational elements of these workloads~(\Cref{sec:model:operational}).

%\vcutM{}
\subsection{Reference Architecture for MLGs}
\label{sec:model:mve-archi}

\begin{figure}[t]
    %\includegraphics[width=.7\linewidth]{figures/MVE Architecture.pdf}
    \includegraphics[width=1\linewidth]{figures/MVE_Architecture.pdf}
    \vcutL{}\vcutS{}
    \caption{Overview of an \mve.} % The explicit network protocol~(\designref{4}) and the explicit state model~(\designref{5}) extend the state-of-the-art.}
    \label{fig:mve}
    \vcutL{}
\end{figure}

%Earlier work defines a high-level reference architecture for \mves~\cite{yardstick} (see Figure~\ref{fig:mve}). 
We leverage in this work a common reference architecture for \mves~\cite{yardstick}.
%Figure~\ref{fig:mve} depicts this reference architecture, which 
% We extend it in this section with an explicit network protocol (component~\designref{4}) and an explicit state model~(\designref{5}). 
%
% In this section we present a reference architecture for \mves, based on existing work~\cite{yardstick}.
% This architecture, shown in Figure~\ref{fig:mve}, describes the main components of an \mve and their interactions.
%
%Overall, 
As Figure~\ref{fig:mve} depicts,
\mves use a client-server architecture and are commonly deployed in cloud environments.
Players run a client on their own device, which connects to a server instance running in the cloud.
Some \mve developers publicly distribute their server software, allowing players to self-host game instances.
Popular cloud providers such as Amazon~AWS and Microsoft~Azure provide tutorials for running these servers on their platform.
Microsoft, the company that currently owns Minecraft, markets it as a cloud-based service through \emph{Minecraft Realms}, which offers players a fully-managed Minecraft instance for a monthly fee~\cite{Realms}.
Additionally, many smaller companies offer \mves as a service; an extensive %incomplete 
list appears in %of such companies is available 
%in our technical report~\citeanon{techreport}.
\Cref{sec:experimental_setup}.

The client~(\designref{1}) has two main tasks. First, it translates player input into in-game actions, which it speculatively applies to the local state and also sends to the server for validation.
The client-server communication uses an implementation-specific protocol~(\designref{4}) that can be shared between different \mves.
Second, the client visualizes the game state, at a fixed rate.
% renders the game state for visual display to the player, at a fixed frequency.

% The client and server communicate via an implementation-specific protocol~(\designref{x}).
% We refer to \mves that implement the protocol used by Minecraft as \mves.
% In Minecraft specifically, the format of both the player actions and state updates are defined in a network messaging system called the \emph{Minecraft protocol}. Third parties have implemented alternative versions of the server that utilize the Minecraft protocol, creating Minecraft-like games that are compatible with the Minecraft client. We utilize three popular Minecraft-like games that implement the Minecraft protocol in our experiments.

The server~(\designref{2}) is responsible for performing all in-game~(virtual-world) simulations, maintaining the global
state, and disseminating state-updates to clients.
Different from simulators in science or engineering, video game simulations tolerate (temporary) inconsistency, and must support modifying the environment via user input.
The \emph{game loop}~(\designref{3}) performs simulations, by applying state-updates to the global state in discrete steps (\emph{ticks}), at a fixed frequency.
In \mves, this frequency is typically set to 20\,Hz, or 50\,ms per tick.
If a tick takes under 50\,ms, the \mve waits for the next scheduled tick start. However, if a tick exceeds 50\,ms, the tick frequency drops below 20\,Hz and the server enters an \emph{overloaded} state.
While in this state, \textit{the game fails to meet its \qos requirements} and can cause players to experience game stuttering, visual inconsistency, % (e.g., \emph{rubber-banding}, where elements of the game appear to sporadically teleport), 
and increased input latency.
Prior work has shown direct causality between increased input latency and reduced player experience~\cite{claypoollatency, unplayable118ms, latency60ms}.

\mves generate workloads, both data- and compute-intensive, that do not exist in other types of games.
In contrast to traditional games, \mves allow modifications to the terrain.
% This but this feature creates a performance challenge.
This requires the game server to simulate terrain changes and manage terrain-state alongside the player- and entity-state found in traditional games~(\designref{5}).
%In contrast to 
Unlike
other types of state, %when the virtual world is large, 
terrain state can be both \textit{data-intensive} and \textit{compute-intensive}, without direct player input.
%because it can change without direct player input.
% Since the environment is not static, it is necessary to continuously calculate the state of the environment and maintain state consistency between players. 
% Additionally, environment simulation rules allow the MVE to modify itself. The environment state is contained in a terrain data-structure~(\designref{4}) that keeps track of each voxel, and that is concurrently accessed during game processing.


\subsection{Workloads in MLGs}\label{sec:Workloads}\label{sec:model:workloads}
\begin{figure}[t]
    \includegraphics[width=\linewidth]{figures/WorkloadModelRemade}
    % \vcutL{}\vcutS{}
    \caption{Workload components in \mves.}
    \label{fig:workloads}
    \vcutM{}%\vcutM{}
\end{figure}

This section presents our workload model for \mves, which focuses on players, terrain, and entities.
%We differentiate in this model three main components of \mve workloads: players, terrain, and entities.
% Figure~\ref{fig:workloads} presents a visual overview of our model.
We discuss each of these components, in turn, focusing on unique and challenging aspects.
%aspects that are either unique to or more challenging for \mves.
%We mark the novel aspects introduced by our research. % with ``novel''.
We distinguish %between known and 
novel aspects in our research.

Figure~\ref{fig:workloads} presents a visual overview of our model.
Beyond the state-of-the-art, our workload model captures \emph{\envworkloads}, which are caused by simulating the modifiable environment itself, and scale independently from the number of active players. We argue \envworkloads are an important part of representative benchmarking workloads for \mves. However, existing benchmarks do not include this type of workload. Addressing this gap, we propose an \mve workload model which describes a wide range of \envworkloads. In Figure~\ref{fig:workloads}, Terrain Simulation and Entities are examples of \envworkloads. %such workloads.


% Together, Terrain Simulation and Entities form \emph{\envworkloads}.
% These workloads are caused by simulating the modifiable environment itself, and scale independently from the number of active players.

\subsubsection{Workload from Players~(known)}
\label{sec:model:workload:players}

Players cause workload for \mves, and games in general, through their actions.
\mves support player-actions found in traditional games, e.g., player movement and interactions, and also \textit{\mve-specific actions}, e.g., to modify terrain.
For player movement, the game computes collisions to prevent players from walking through obstacles such as walls, and disseminates location-changes to other players.
Players can also interact with other players and entities (i.e., objects), for example by collecting resources and exchanging them with other players.

An important difference between \mves and traditional games is support for player-actions that modify the terrain.
% movement to previously unexplored sections of the game world causes the generation of new terrain, and players can destroy and create voxels. 
In \mves, players can \textit{terraform}---create, modify, and destroy the terrain, as well as the buildings standing on the terrain.
%---by, for example, constructing and removing buildings, mountains, and rivers.
This can generate resource-intensive workloads in two ways.
First, players can change a large part of the terrain in a short amount of time, for example through the use of explosives.
This is both compute- and data-intensive, because the game needs to compute the new terrain, and communicate state updates to keep a consistent view across all players.
Second, players can construct dynamic elements such as \emph{simulated constructs}, which increase the complexity of the terrain simulation
and are discussed in~\Cref{sec:model:workloads:environment}.
The impact of player workloads has been previously examined in both the context of traditional video games architectures and \mves specifically~\cite{MMOPlayersWorkload,yardstick}.

%However, we identify a novel type of player behavior unique to Minecraft-like games that results in complexity scaling separate from player count. Through specific terrain modifications, players can create structures that utilize environment simulations rules to form complex automata, using certain voxels to act analogously to sensors, actuators and wires. We call the player behavior to create such constructs \emph{player-defined logic} and the constructs themselves \emph{simulated constructs}. 
%Player-defined logic is often an intentional feature designed to allow the player to construct \emph{resource farms}: simulated constructs that automate the generation or collection of in-game resources. Some Minecraft-like games specifically facilitate player-defined logic, such as by providing voxels that act as circuitry, or methods of duplicating simulated constructs. Minecraft itself provides a comprehensive logic system specifically for the construction of simulated constructs, known as Redstone~\cite{minecraftlogic}. Other examples include Conveyor~\cite{satisfactorylogic} systems in Satisfactory, Wire~\cite{terrarialogic} in Terraria, Circuits~\cite{factoriologic} in Factorio, Modules~\cite{astroneerlogic} in Astroneers, and Logic~\cite{nomansskylogic} in No Man’s Sky. However, even in games that do not explicitly support player-defined logic, it is still possible for players to create simulated constructs though applying knowledge of environment simulation rules. Since the behavior of simulated constructs is defined through structure, the only limit to their computation complexity is maximum environment size. The simulations rules of some Minecraft-like games have even been proven to be Turing complete~\cite{redstoneturing}, allowing for the creation of simulated constructs that behave as functional computer systems.

%Simulated constructs add additional environment computation to the game loop, independent on continued interaction from players. Simulated constructs, as groups of voxels within the terrain, will be processed via environment simulation rules for the duration the server is operating, even if the player who created the construct is no longer connected to the server. 
%Thus, the act of creating a simulated construct itself does not directly create higher workload complexity beyond typical player actions that modify terrain. Instead, it is the behavior of the simulated constructs that increases computational complexity. 
%Accordingly, simulated constructs are an example of \envworkloads.



\begin{figure*}[t]
    \includegraphics[width=\textwidth]{figures/Operational_Model.pdf}
    \vcutL{}
    \caption{Operational model of an \mve. Note different elements of the Game Loop can be run concurrently.}
    \label{fig:operational}
    \vcutM{}
\end{figure*}

\subsubsection{Workload from Terrain Simulation~(novel)}
\label{sec:model:workloads:environment}

In contrast to traditional games, a significant part of the \mve workload can come from generating and simulating the terrain.
\mves typically present players with an endless open world.
This \textit{world} is split into areas, which are lazily generated when players come near them.
Once the terrain is generated, the game simulates it and allows players to modify it.


We identify four important components of terrain simulation: physics, lighting, plant growth, and simulated constructs.
Although \textit{physics and lighting} simulations are present in traditional games,
the modifiable nature of the terrain makes it significantly more challenging to manage such features in \mves.
Unlike static environments, where physics simulation only needs to happen for the relatively few entities that can move through the world, \mves need to perform physics simulations on the many blocks that compose the terrain itself.
For example, a bridge can collapse when a player removes its support pillars, or the terrain underneath them.
Once the bridge has collapsed, the bridge no longer casts shadow, so the simulator needs to recompute lighting (frequently) at runtime; static environments do not have this dynamic workload.
%In contrast, static environments require terrain lighting to be performed only once.

\textit{Plant growth} is an example of a dynamic element unique to \mves. %which does not exist in static environments.
%In modifiable worlds, plants 
Plants and trees change over time, reshaping the nearby terrain, thus generating new workload.
%This generates additional workload in \mves.
%% These simulations require additional resources from the game and create additional workload.

% After terrain has been generated it then must be simulated. Minecraft-like games define a set of simulation rules that determines how voxels states will change over time. Each rule consists of an activation condition and resulting modification to voxel properties. %Depending on the purpose of the rule, the activation condition may be gated with a random number generator to cause the rule to activate at random intervals, or be tied a timer to activate with delay or at a frequency longer than one tick. 
% These rules are used to add dynamism to the environment and perform physics simulations, such as by defining the spread of `liquid' voxels, the effects of gravity, real-time lighting, and the growth of plants.

%In a single tick, any amount of rules can be activated, and the method of deciding the order of rules to execute varies for each Minecraft-like game. Similarly, the resolution of a given rule can trigger the activation of another, creating the possibility for rule execution stack-overflows. In practice, Minecraft-like games avoid overflows by forcefully ending a tick or delaying execution of a rule to future ticks.

% Generally, the area within the environment that activates a simulation rule is also the area that is modified by that rule, giving environment simulations the property of \emph{spatial locality}. In areas where %simulation rules activate at a low frequency, the state of the environment is stable, causing simulation rule activation frequency to tend to remain low, but in areas where
% rule activations are more rapid, environment state updates occur at a correspondingly faster rate, causing more opportunities for further rule activation. This means that relatively small sections of the game world can contribute to a disproportionately high percent of the game workload.

% With knowledge of these rules, players can create structures that utilize environment simulation rules to form complex automata, using certain voxels to act analogously to sensors, actuators and wires. We call the player behavior to create such constructs \emph{player-defined logic} and the constructs themselves \emph{simulated constructs}. 

Through terrain modification, players can create \emph{simulated constructs}.
In a simulated construct, players place together dynamic elements (e.g., plants, automatic croppers) to achieve a certain goal.
For example, many players build irrigation systems that grow and harvest vegetables automatically, with high yield.
%Such systems require a deep understanding of the game rules, and depend on the interaction of many dynamic elements,
Such systems can leverage tens to hundreds of dynamic elements,
whose interaction generates compute-intensive workload for terrain simulation.
%and increases the computational complexity of the terrain simulation.

% Player-defined logic is often an intentional feature designed to allow the player to construct \emph{resource farms}: simulated constructs that automate the generation or collection of in-game resources. Some Minecraft-like games specifically facilitate player-defined logic, such as by providing voxels that act as circuitry, or methods of duplicating simulated constructs. Minecraft itself provides a comprehensive logic system specifically for the construction of simulated constructs, known as Redstone~\cite{minecraftlogic}. Other examples include Conveyor~\cite{satisfactorylogic} systems in Satisfactory, Wire~\cite{terrarialogic} in Terraria, Circuits~\cite{factoriologic} in Factorio, Modules~\cite{astroneerlogic} in Astroneers, and Logic~\cite{nomansskylogic} in No Man’s Sky. However, even in games that do not explicitly support player-defined logic, it is still possible for players to create simulated constructs though applying knowledge of environment simulation rules. Since the behavior of simulated constructs is defined through structure, the only limit to their computation complexity is maximum environment size. The simulations rules of some Minecraft-like games have even been proven to be Turing complete~\cite{redstoneturing}, allowing for the creation of simulated constructs that behave as functional computer systems.

\textit{In \mves}, as we show in~\Cref{sec:experiments}, \textit{even a single player can overload the game simulator.}
This is in part because, in \mves, a single player can trigger complex simulations, for example, by building simulated constructs of arbitrary size.
By contrast, in traditional games, only the number of concurrent players is strongly correlated with workload intensity.

% Interestingly, a single player can create simulated constructs of arbitrary size, creating a more complex relationship between
% the number of players in the game and the intensity of the game's workload.
% In our model (and in practice, as we show in~\Cref{sec:experiments}) a single player can cause an \mve to become overloaded.

% Simulated constructs add additional environment computation to the game loop, independent on continued interaction from players. Simulated constructs, as groups of voxels within the terrain, will be processed via environment simulation rules for the duration the server is operating, even if the player who created the construct is no longer connected to the server. 

%\vcutS{}
\subsubsection{Workload from Entities~(novel)}

An \emph{entity} is an object that exists in the virtual world but is not a player or terrain.
Examples include \npcs, mobiles (i.e., \emph{mobs}), and items (e.g., a sword).
Entities can typically move or be moved by players and collide with each other.
Here we describe two important aspects of entity simulation which are challenging for \mves.
% Similar to physics simulation and lighting in terrain simulation, entities also exist in traditional games,
% but are more challenging to support in \mves due to the modifiable terrain.

First, games typically instantiate entities at \emph{spawn points}, e.g.,
spawn an \npc at a spawn point in a dark cave when a player is about to enter.
% spread throughout the world.
%For example, the game may spawn an \npc at a spawn point in a dark cave when a player is about to enter.
In contrast to static environments, where game developers typically place these spawn points manually, \mves need to compute spawn points dynamically
%because 
as
terrain modification may obstruct existing spawn points.

Second, \npcs use path-finding algorithms to move around the map.
Static worlds pre-compute overlay graphs with viable \npc locations,  improving computational efficiency.
In contrast, \mves have changing terrain, so they must compute path-finding graphs dynamically, leading to additional compute-intensive workload.
%%In \mves, path-finding graphs must be computed dynamically to address  changing terrain, making \npc movement more computationally expensive. % than in traditional games.

% Additionally, some entities have the ability to modify terrain, creating additional complexity when performing decision calculations.

% Entities exist in games that are not Minecraft-like, but MVEs have unique properties that change how entities behave in Minecraft-like games which generally make them less efficient to compute.

% In a modifiable world there are no set locations for entities to spawn, thus continuous calculations are performed to determine when and where an entity should appear. Similarly, entity decision algorithms for actions such as path-finding and terrain modification cannot make use of  ``checkpoint'' systems to pre-calculate paths and actions as is done in games without MVEs. Additionally, such action calculations must be repeated each time the surrounding game state changes. 

%Within this definition, there are a few main classes: \textit{driven entities} exhibit some form of decision making and movement ability (often referred to as ``\textit{mobs}"), and \textit{non-driven entities}, which generally represent an in-game resource or provide some functional or visual effect. Driven entities often take the form of humans or animals, and notably can have the ability to alter the terrain of their own accord. All driven entities require access to environment state in order to perform decision making and pathfinding.

%There are also wide variety of non-driven entities common in Minecraft-like games, such as dropped items, vehicles, and weapons. These entities generally exist to be interacted with, moved or used. While they have no decision capability, they still require computation for collision and movement.

%\vcutS{}
\subsection{Operational Model of \mves}
\label{sec:model:operational}

We detail in this section the game loop used by \mves.
We
define the \emph{operational model} as the set of operations, and of events triggering and linking them, of individual components in the  implementation of the game loop.
Novel, in this work, we analyze the performance implications of the unique aspects of \mve workloads~(see~\Cref{sec:model:workloads}) when executed with the \mve operational model.

Figure~\ref{fig:operational} depicts a constructed, generalized, and simplified operational model of the \mve game loop. %%the game loop of a generalized \mve.
 To run the game loop, the game server orchestrates primarily three main components, the
Networking Queues~(component~\designref{1} in Figure~\ref{fig:operational}), the Game Loop~(\designref{2}), and the Game State~(\designref{3}), which we discuss in turn.
%In the remainder of this section, we discuss their internal processes and interactions.

% through an example.


% to coordinate components across client and server, through an example. Because the game loop and the protocol are implementation-specific, we refer to each specific implementation as an \emph{operational trace} of a specific \mve.

% Overview, top-level components
% In Figure~\ref{fig:operational} we show an example trace of the game loop of a generalized \mve.
% The game loop runs on the game server, the latter of which has three main components:
% Networking Queues, the Game Loop, and the Game State.
% In the remainder of this section, we discuss their internal processes and interactions.

The Networking Queues~(\designref{1}) buffer between the game clients and the server.
When a client sends a player-action to the server, it is buffered in the incoming network queue until the next tick.
When the server needs to send a state-update to one or several clients,
it forwards the message to the networking queues, to be further buffered in the outgoing queue or sent directly to the client.

The Game Loop~(\designref{2}) simulates the virtual world and is the core of the game server.
% The Game Loop~(\designref{2}) simulates the virtual world and is the core of the game server.
In an \mve, the game loop consists of three elements: players, the terrain, and entities. These elements correspond to the workloads specified in~\Cref{sec:model:workloads}.
Figure~\ref{fig:operational} shows each of these elements, and how they differ from the others.
For each element, its simulation typically requires reading the current game state~(\designref{3}), and may result in terrain state changes that need to be persisted~(i.e., written).
In this section, we focus on the terrain state because it is idiosyncratic to \mves.
Below, we discuss each simulation element in turn.


% The operation of \mves has two main steps that are executed sequentially: processing player, entity, and terrain changes (Game Loop,~\designref{1}), and sending the resulting state updates to players (Network Queue Out,~\designref{2}). 
%The processing step is known as a \emph{tick}, and is defined as one iteration of the game logic loop. 
% The specific computations performed within each tick form the \emph{workload} of the server. Depending on the amount and complexity of actions within the workload, the duration of each tick changes. As the sending of state updates to players can only be done once a tick has finished, this tick duration also decides the frequency of state updates to players. 

% Players
The Player Handler~(\designref{4}) is driven by player actions, which the Game Loop retrieves from the Networking Queues once per tick.
% The Game Loop  retrieves any player actions from the network once per tick.
For example, players can move or build something in the virtual world.
Because the terrain can obstruct the player from performing these actions, the Player Handler must read the terrain state in the vicinity of the player.
If the action is successful, player actions that affect the terrain (e.g., building) need to be written back to the global Game State.

% Terrain
Terrain Simulation~(\designref{5}) is largely independent from player input, and is instead driven by terrain state updates. When a terrain state update occurs, the Terrain Simulation applies its simulation rules to the new state. For example, a terrain simulation rule such as \emph{if terrain is not physically supported, it falls down} can be triggered when a player removes the keystone from a bridge. These rules trigger in a loop, where each iteration informs the adjacent terrain that it is no longer supported. The resulting state changes are written back to the global Game State.

% Entities
Entities~(\designref{6}) are primarily driven by the Game State, including the state of the terrain, players, and entities themselves.
% Entities are primarily driven by the Game State, including the state of the terrain, players, and entities themselves.
Entities such as \npcs need the terrain state primarily for pathfinding. In some cases, entities may themselves modify the terrain. For example, an \npc may place or remove terrain, or items such as explosives may remove large parts of terrain all at once.

Although, from a performance perspective, it is desirable to run the game loop elements concurrently,
there are two challenges with this approach.
First, while these elements are in principle independent, they have implicit dependencies through the game state which they access.
Individual elements can only run concurrently as long as they do not access the same state.
Second, terrain simulation rules can cause a sequence of state changes which cannot be parallelized, as is the case in the bridge example above.

Using our operational model for \mves, we formulate two implications for \mve performance variability.
First, because \envworkloads do not rely on the presence of players, large \envworkloads can cause ticks to exceed their maximum duration,
even with few or no players connected.
Second, because player simulation and \envworkloads must be completed sequentially when they access the same state,
even small \envworkloads can affect tick duration given they are spatially clustered.



==> TECHNICAL REPORT ICPE2023 Meterstick NEW/content/3_benchmark_design.tex <==
\section{\toolname Benchmark Design}
\label{sec:design}\label{sec:system-design}

To address contribution~\ref{contrib:design}, we design \toolname, a benchmark for evaluating performance variability in \mves. The main novelty of \toolname relates to its workloads (\Cref{sec:benchmark_workloads}) and performance metrics (\Cref{sec:design:metrics} and~\Cref{sec:metric}).

\subsection{System Requirements} \label{sec:requirements}

Here we describe our eight requirements for \toolname.
We define the first three requirements specifically for our use case.
The last five relate to benchmarking computer systems in general, and are based on existing guidelines~\cite{DBLP:conf/performance/Weicker02, performanceanalysis}.
\begin{enumerate}[label=\textbf{R\arabic*}]
  \item\label{req:capture-variability} \textit{Captures performance variability of \mves:} \toolname must be capable of capturing relevant performance metrics at a granularity sufficient for analysis of variability. The specific measure of variability must be applicable and meaningful in the context of \mves.

  \item\label{req:valid-workloads} \textit{Validity of workloads:} The workloads used in benchmarking of the \mve should be representative of real-world use and address the workload types listed in~\Cref{sec:Workloads}.

  \item\label{req:extensive-exps-and-metrics} \textit{Relevant metrics and experiments:} The benchmark should support relevant experiments to isolate different sources of variability, and collect meaningful metrics to allow suitable analysis of these sources.

  \item\label{req:fairness} \textit{Fairness:} The benchmark should provide a fair assessment for compatible systems. In particular, bias towards any one system should be limited.

  \item\label{req:easeofuse} \textit{Ease of Use:} The benchmark should be easy to configure and use with any compatible system.

  \item\label{req:clarity} \textit{Clarity:} The benchmark should present results to the user in a way that is suitable for system performance variability.

  \item\label{req:portable} \textit{Portability:} The benchmark should support common deployment environments and be easy to port to others.

  \item\label{req:scalability} \textit{Scalability:} Benchmark workloads should be scalable to accommodate benchmarking on increasingly powerful hardware or with more performant systems.
\end{enumerate}

\begin{figure}[t]
  \includegraphics[width=.9\linewidth]{figures/Benchmark_Design_Anon.pdf}
  \vcutM{}
  \caption{Architecture of \toolname. Component \designref{6} is system under test. Component \designref{5} adapts tool~\cite{yardstick}.}
  \label{fig:benchmark}
  \vcutL{}
\end{figure}

\subsection{Design Overview}
Here we present the design of \toolname, our system for benchmarking of performance variability in \mves.
%A list of guiding design requirements is available in the technical report~\citeanon{techreport}.
Figure~\ref{fig:benchmark} presents \toolname's high-level design.
% overview of \toolname in Figure~\ref{fig:benchmark}.
We discuss the benchmark workloads~(addresses \textbf{R2}) and metrics~(partially addresses~\textbf{R3}) in more detail in~\Cref{sec:design:workloads} and~\Cref{sec:design:metrics} respectively.

% We discuss the benchmark workloads and metrics in more detail in~\Cref{sec:design:workloads} and~\Cref{sec:design:metrics} respectively.

% As we design a benchmarking tool, we additionally define a benchmarking technique, which includes the experiment configuration~(\Cref{sec:Configuration_Parameters}) and metrics~(\Cref{sec:metrics}).

% Configuration, component 1, R1
% In our design, the user mainly interacts with \toolname through its Configuration component~(\designref{1}).
% The Configuration allows the user to capture performance variability by specifying the duration and number of iterations of experiments~(partially addresses~\ref{req:capture-variability}).
% The Configuration further allows users to configure benchmark parameters, such as the systems under test and workload, and deployment parameters, such as machine IP addresses~(partially addresses~\ref{req:easeofuse}).

In our design, the user mainly interacts with \toolname through its Configuration component~(\designref{1}).
The Configuration allows the user to capture performance variability by specifying the duration and number of iterations of experiments~(partially addresses~\ref{req:capture-variability}).
The Configuration further allows users to configure benchmark parameters, such as the systems under test and workload, and deployment parameters, such as machine IP addresses~(partially addresses~\ref{req:easeofuse}).
%\info{R4C5}

% Deployment, component 2
After specifying the configuration, the user launches \toolname.
This triggers the Deployment component~(\designref{2}), which deploys components and software dependencies to remote machines specified in the configuration.
This only requires the user needs to specify a set of IP addresses of \texttt{ssh}-accessible machines.
This makes \toolname portable~(\ref{req:portable}),
and allows users to evaluate \mve performance variability under cloud or self-hosted deployments.
% For example, the user can configure the player emulation to run in a different geographical location than the \mve to evaluate performance variability when players connect over the Internet~(partially addresses~\ref{req:extensive-exps-and-metrics}).

% Control server, component 3
When deployment is complete, the Deployment component hands control to the Control Server~(\designref{3}).
\toolname follows a Controller/Worker pattern,
with the Control Server as the controller, and the Control Clients as the workers~(\designref{4}).
The Control Server contains the operation logic, and is responsible for synchronizes the operation of all workers by exchanging messages with each Control Client running on each worker. The Control Server and Clients exchange the messages enumerated in Table~\ref{tab:cont_messages}.
% Control client, component 4
Depending on the configuration, the Control Client runs either \emph{player emulation} or the \mve.

% MVE and Yardstick, components 5+6
\toolname uses one or more workers for player emulation~(\designref{5}).
These workers emulate players by connecting the \mve and automatically sending player actions based on programmed behavior. \toolname implements this by using the player emulation from Yardstick~\cite{yardstick}, an existing \mve benchmark which we compare to \toolname in detail in~\Cref{sec:related-work}.

% Metrix Externalizer + System Metrics Collector, component 7+8
One worker runs the \mve~(\designref{6}), which is the system under test.
\toolname captures the \mve's performance variability metrics using the player emulator (\designref{5}), the metric externalizer~(\designref{7}), and the system metrics collector~(\designref{8}).
%We detail 
\Cref{sec:design:metrics} details
the operation of these components and the metrics they collect, including our novel metric to capture performance variability. %, in~\Cref{sec:design:metrics}.

% Data retrieval + Data visualization, component 9+10, R6
When the benchmark experiments are done, the Control Server activates the Data Retrieval and Data Visualization components~(\designref{9} and \designref{10}),
This component moves the collected data from the worker nodes to the user's local machine, where it pre-processes the data through aggregation and reformatting.
The Data Visualization component~(\designref{10}) takes as input the processed data and automatically outputs 
producing basic plots for \mve performance and performance variability.
Users can view these plots, and, if desired, provide their own advanced plotting scripts for in-depth analysis
~(concludes~\ref{req:easeofuse},~\ref{req:clarity}).
\begin{table}[t]
  \begin{center}
    \caption{List of controller messages. Dest specifies what nodes the message is for where Y is player emulation, M is the server node and C is the controller.
    \label{tab:cont_messages}}
    \begin{tabular}{l l c}
      \hline
      \textbf{Message} & \textbf{Effect} & \textbf{Dest}\\
      \hline
       set\_server:\textit{server} & Specifies name of server & Y/M\\
       set\_jmx:\textit{jmx url} & Specifies JMX URL & M\\
       iter:\textit{iteration} & Specifies what iteration to start at & Y/M \\
       initialize & Starts the selected server & M\\
       log\_start & Starts metric logging tools & M\\
       log\_stop & Stops metric logging tools & M\\
       stop\_server & Stops running server & M\\
       connect & Starts player emulation & Y\\
       convert & Converts metric bin files to CSV & Y \\
       ok & Acknowledges the previous message & C\\
       keep\_alive & No-op, keeps TCP connection open & M/Y\\
       err:\textit{error} & Previous message has caused error & C\\
       exit & Stops the controller client & M/Y\\
      \hline
    \end{tabular}
  \end{center}
\end{table}

% Misc
% The deployment tool and the controller server and clients allow for remote operation of benchmark components within distributed environments, and are generalized to operate on any modern commercial cloud, making \toolname portable (\textbf{R7}). Additionally, as \toolname supports testing of any \mve that uses the Minecraft network protocol and supports the metric externalizer instrument (\designref{7}, see \Cref{sec:design:metrics}), \toolname provides fair comparison of \mve systems (\textbf{R4}) and is easily extensible to new ones (concludes~\textbf{R5}).

\subsection[Benchmark Workloads]{Benchmark Workloads
  (address \ref{req:valid-workloads},~\ref{req:fairness},~\ref{req:scalability})
}\label{sec:benchmark_workloads}
\label{sec:design:workloads}
% In this section, we outline our selection criteria for representative workloads~(\textbf{R7}) and the resulting choice in benchmark workloads.
This section presents \toolname's workloads.
\toolname uses the workload model presented in \Cref{sec:model},
which divides workloads in three main components: \emph{players}, \emph{terrain simulation}, and \emph{entities}.
By using this model, \toolname's workloads are applicable to \mves in general, thus avoiding favoring specific systems (partially addresses~\ref{req:fairness}).
In practice, the user specifies in the Configuration~(\designref{1}) only the \emph{player} and \emph{terrain simulation} parts of the workload,
as \emph{entities} are a result of terrain simulation (spawning, see \Cref{sec:Workloads}).

As future systems may become sufficiently performant to mitigate the impact of \toolname's workloads, \toolname supports workload scaling~(\ref{req:scalability}).
To increase \toolname's workload complexity, the user can specify an increased number of players to scale the player workload, and use \toolname's \emph{scale} parameter to select higher-complexity versions of the pre-configured workloads.

While \toolname supports arbitrary valid Minecraft worlds as workloads, the remainder of this section describes the workloads we design for use in our experiments to highlight performance variability based off our workload model and observable community use~(\ref{req:valid-workloads}).

The conceptual challenge of designing the benchmark workloads stems from the vast design space. \mves give players fine-grained control over the virtual environment,
resulting in an endless number of possible world permutations and a large variety in types of simulated constructs.

Additionally, finding evidence to support our selection proved to be challenging, as no peer-reviewed analysis of such artifacts currently exists and game operators do not want to share such information; searching for trustworthy communities and identifying suitable artifacts poses additional challenges. We detail our workload design and the evidence supporting it throughout this section.

\subsubsection{The Environment-Based Workloads}\label{sec:environment_workloads}
The environment workload is determined by the \mve's terrain generation and the terrain modifications made by players.
%Benchmarks should use representative workloads which capture essential features of community use.
To obtain representative worlds and workloads, we reconstruct highly popular creations (templates of useful simulated constructs, see~\Cref{sec:model:workloads}) available on common sharing platforms in the \mve community.
Because the \mve community thrives on sharing player-created content with other players, this approach captures essential features of how the community uses these systems.


To cover the range of valid workloads~(\ref{req:valid-workloads}),
we include two worlds that result in a best-case workload and worst-case workload respectively.
During all \envworkloads, \toolname connects to the game a single player that performs no actions.
This is necessary to correctly capture the response time metric discussed in \Cref{sec:metrics}.
The remainder of this section describes the worlds and their resulting workloads.
% worlds that contain examples of environment workloads as defined by our workload model in \Cref{sec:Workloads}. 
% Where applicable, we choose specific designs of environment workloads from popular community sources, to ensure that they are representative~(\textbf{R7}). Additionally, to ensure we sufficiently cover the range of possible workloads(\textbf{R2}) we include a best-case workload in the form of the Control workload and have the Lag workload as a worst-case. 
We list the worlds used in Table~\ref{tab:worlds}.

\begin{table}[t]
  \begin{center}
    %\caption{Worlds containing environment workloads defined in \toolname benchmark.
    \caption{Minecraft worlds used as workload starting points by the \toolname benchmark.}
    \label{tab:worlds}
    \begin{tabular}{l l r}
      \toprule
      \textbf{Name} & \textbf{Properties}                      & \textbf{Size [MB]} \\
      \midrule
      Control       & Freshly generated world                  & 5.4                \\
      TNT           & Entity actions, terrain updates          & 6.3                \\
      Farm          & Resource Farm constructs                 & 26.0               \\
      Lag           & Complex simulated construct, stress test & 4.7                \\
      \bottomrule
    \end{tabular}
  \end{center}
  \vcutL{}
\end{table}

\begin{table}[t]
  \begin{center}
    \caption{Simulated constructs in Farm world and their author. Popularity measured in millions of views.
    \label{tab:farmconstructs}}
    \begin{tabular}{l r l c} 
      \toprule
      \textbf{Name} & \textbf{Amount}& \textbf{Author}& \textbf{Popularity}\\
      & & & [$10^6$ views] \\
      \midrule
      Entity Farm &12&gnembon~\cite{ytmobfarm} & 1.7\\
      Stone Farm &4&Shulkercraft~\cite{ytcobblefarm} & 1.3\\
      Kelp Farm &4&Mumbo Jumbo~\cite{ytkelpfarm} & 2.5 \\
      Item Sorter &1&Mysticat~\cite{ytitemsort}& 0.8 \\
      \bottomrule
    \end{tabular}
  \end{center}
\end{table}

% As we are measuring the impact of environment, rather than player, workloads, we connect only a single player that stands still in each experiment.
% We use this player's network message data during the computation of game response time.

The Control world results in a best-case workload while still being realistic.
The Control world is an unmodified world %similar to those encountered by players that start a new game.
%The world is 
generated by Minecraft version 1.16.4 using the seed -392114485.
The measured results of this workload are used as a workload-level baseline to compare the other workloads.

The TNT world contains a 16-by-16-by-14 cuboid filled with TNT blocks which are set to explode around 20 seconds after a player connects.
In the systems tested, TNT operates by spawning an entity, which can be interacted with by other entities, including other TNT entities. Thus, when a large section of TNT is activated, the \mve must perform a large number of both entity-collision and physics calculations.
Intentionally creating large-scale TNT chain reactions is a popular activity, which can be observed in a plethora of community-made content. For example, a video from 2018 that shows a chain reaction of thousands of TNT blocks has 21~million views~\cite{yttnt}.

The Farm world contains multiple \emph{resource farms}, which are simulated constructs built by players to automatically generate in-game resources. The specific designs of the simulated constructs in this workload were sourced from popular community creators and each have 1.6~million views on average.
Table~\ref{tab:farmconstructs} gives an overview of all resource farms present in the Farm world, their respective authors and popularity.
 The Farm world has many different resource farm simulated constructs, which we list in Table~\ref{tab:farmconstructs}.
The Entity and Stone farms are %controlled by a `clock' simulated construct which 
activated at a fixed interval of around 4 seconds, whereas the Kelp and Item sorter use event-based activation. 
These farms rely on entities in their functioning, through spawning driven entities and manipulating their pathfinding, or through the creation of passive entities to represent item resources. A core feature of \mves is collection of resources from the game environment. The ability for players to construct simulated constructs that automate this process is both an intended and common behavior.
The Entity farm relies on spawning driven entities and manipulating their movement. The Stone and Kelp farm continuously destroy blocks, which create passive entities to represent items. These item entities are then transported through terrain simulation rules (e.g. liquid physics simulation).

The Lag world results in a worst-case workload.
%This world contains a single \emph{Lag Machine} simulated construct.
This world contains a simulated construct known in the \mve community as a \emph{Lag Machine}.
Lag Machines are a specific subset of simulated constructs that are designed to cause high computational load for the \mve, either for the purpose of stress testing it, or to cause it to crash as part of a denial of service attack.
The design of the Lag Machine used in this workload is publicly available and provided by a community-creator with 52 thousand subscribers~\cite{ytlag}. It is chosen as it operates based on terrain simulation rules. Specifically, it uses many logic-gate constructs in a small area to cause a high volume of simulation rule activations. Importantly, the simulation rules this Lag Machine uses are generally non-malicious, and are used in many resource farm constructs, as well as forming the basis for simulated constructs such as an operational digital Computer~\cite{ytcomputer}.


\subsection{Configuration Parameters} \label{sec:Configuration_Parameters}

\toolname is highly configurable in order to be extensible to new Minecraft-like games, environments, workloads, and experiments~(\textbf{R5}). A list of configuration parameters are given in Table~\ref{tab:parameters}.

\begin{table}[t]
  \begin{center}
    \caption{List of configurable parameters. V, F and P refer to Vanilla, Forge and PaperMC respectively.
    \label{tab:parameters}}
    \begin{tabular}{l l l}
      \hline
      \textbf{Parameter} & \textbf{Specifies}& \textbf{Typical Value}\\
      \hline
      IPs  &  Nodes used & none\\
      SSL Keys  & Authentication & none \\
      Servers & Minecraft-like games & V, F, P\\
      World & World workloads & Control \\
      File Locations & Output directories & /ys/, /mc/\\
      Resume  & Continue experiment & False\\ 
      Ports& Network config & 25555/25565\\
      JMX URLs & Metric collection&Various\\
      JMX Ports&  Metric collection &25585-25635\\
      RAM & RAM (JVM argument) &4GB\\
      Affinity & CPU Affinity & 0xFFFFFFFF\\
      Number of Bots & Player count&25 \\
      Behavior & Player actions&Bounded random\\
      Duration  & Iteration length & 60 seconds\\
      Iterations  & Iteration amount & 1\\
      Scale & Workload intensity & 1\\ 
      \hline
    \end{tabular}
  \end{center}
\end{table}

% By adding servers into the servers folder, new systems can easily be added. Similarly, since the deployment process simply copies the servers folder to the remote node, new world workloads can be added by copying them into the worlds directory. 

The experiment can be configured by specifying the duration, number of iterations, what servers to run, how many players to connect and the behavior of those players. Since the IPs of the nodes that the deployment tool connects to can be anywhere that is network accessible, nodes can be chosen that are geographically distant or within the same datacenter in order to measure (or avoid) the performance impact caused by public network infrastructure.

% Although the benchmark workloads are already computationally intense, future hardware and systems may become sufficiently performant to mitigate their impact. Thus, the TNT, Farm and Lag workloads described in Section~\ref{sec:environment_workloads} are tileable, and can be extended by copying sections of the terrain to achieve a increasing complexity. Provided in the benchmark are versions of these worlds where this copying has been done to relevant sections for double and quadruple complexity versions. The `scale' parameter accepts the values 1, 2 and 4 to decide between these scaled world versions.

\subsubsection{The Player-Based Workload}\label{sec:player_workloads}
\toolname uses a player-based workload facilitated by the player emulation component~(\designref{5}).
% The player contribution to the workload of the server comes from both amount of players and their behavior.
% For reproducible player behavior, we use the player emulation component of the Yardstick benchmark~\cite{yardstick},
% which connects emulated players through the Minecraft protocol to the game server.
In this workload, \toolname is configured to connect 25 players which move randomly in a 32-by-32 area. The existing Yardstick benchmark~\cite{yardstick} focuses solely on the impact of player workload. So, we include this player workload to represent a high-density area in \mves and allow \toolname to compare the impact of \envworkloads with a traditional player-based workload.
% However, to facilitate comparison of the impact of environment and player workloads, we additionally run an experiment with 25 players that use a \emph{bounded random} movement behavior: they continuously move in an area of fixed size (set at 32 by 32 voxels).
We select a player count of 25 based on the Minecraft Wiki's dedicated server recommendation~\cite{serverrequirements}, as well as the recommendations from various commercial cloud providers (see \Cref{sec:experimental_setup}).
% END PLAYER SUBSECTION

\subsection[Metrics]{Metrics
  (address \ref{req:capture-variability},~\ref{req:extensive-exps-and-metrics},~\ref{req:fairness})}
\label{sec:metrics}
\label{sec:design:metrics}

This section describes the \begin{addtext}application-level and system-level metrics \end{addtext} metrics collected by \toolname, selected to fulfill \ref{req:extensive-exps-and-metrics}.
% We first describe
% our novel \emph{\newmetric} which quantifies performance variability
% ~(concludes~\ref{req:capture-variability}).
% Next, we describe 
% the application-level and system-level metrics collected by \toolname.
In ~\Cref{sec:metric} we describe our novel \emph{\newmetric} which quantifies performance variability ~(concludes~\ref{req:capture-variability}).
Our \newmetric metric and all application and system metrics are general to \mves to avoid bias for specific implementations (concludes~\ref{req:fairness}).
Table~\ref{tab:metrics} gives an overview of the collected metrics.

\begin{table}[t]
  \begin{center}
    % \caption{Metrics collected by \toolname. Src is source of the metric, where M is Minecraft-like game server, C is the clients, S is system, and D is derived.}
    \caption{Metrics collected by \toolname. The metric type is \underline{D}erived, \underline{A}pplication level, or \underline{S}ystem level.}
    \label{tab:metrics}
    \vcutS{}
    \begin{tabular}{l l l r}
      \toprule
      \textbf{Type} & \textbf{Metric}   & \textbf{Description}                          \\
      \midrule
      D             & \newmetricfull    & Tick instability (see~\Cref{sec:metric}) \\
      \midrule
      A             & Response time     & Round trip latency for clients                \\
      A             & Tick duration     & Duration of each tick                         \\
      A             & Tick distribution & Tick time by workload                         \\
      %   \hline
      %   Messages & A & Timestamp, contents of messages\\
      \midrule
      S             & CPU               & CPU utilization                               \\
      S             & Memory            & Memory usage                                  \\
      S             & Threads           & Thread total                                  \\
      S             & Disk I/O          & Bytes read/written                            \\
      S             & Network I/O       & Bytes sent/received                           \\
      %   Tick magnitude & D & Mean tick duration\\
      \bottomrule
    \end{tabular}
  \end{center}
  \vcutL{}
\end{table}

\subsubsection{Application-level Metrics}
\label{sec:design:metrics:application}

\toolname collects three application level metrics:
% the Yardstick Player Emulation and the Metric Externalizer.
% While the main responsibility of the Yardstick Player Emulation~(\designref{5}) is to emulate players in the \mve,
% its secondary responsibility is to capture message traces sent between the emulated players and the \mve server.
% The message traces give \toolname users the option to perform in-depth analysis analysis on the game's behavior,
% and allows \toolname to derive the \emph{response time} metric, described in \Cref{sec:design:metrics:derived}.
\emph{response time}, \emph{tick duration}, and \emph{tick distribution}.

Response time is how system latency becomes visible to the user.
Lower values are better, and we use existing latency thresholds for the game becoming noticeable and unplayable at 60ms and 116ms respectively~\cite{latency60ms,unplayable118ms}.
% \info{R3C4, R3C5}

The response time is measured as the time between a player taking an action and the results of that action becoming visible.
During this time, the action is sent over network to the \mve server, added to an input queue, simulated during the next tick, has its resulting state changes added to the output queue, and then sent back to the client over the network. In our workload model (Figure~\ref{fig:operational}), this is visible as the time difference between the client sending player actions (\designref{A}) and receiving state updates (\designref{C}).
\toolname captures this metric by having a player send \emph{chat} messages to all players (including itself), and measuring how long it takes for the player to receive its own message.

While tick duration and tick distribution cannot be directly observed by players,
\mves typically expose these metrics through interfaces commonly used by debugging tools.
\toolname's Metric Externalizer~(\designref{7}) uses these interfaces to gain access to these metrics without requiring access to the game's source code.
As a consequence, \toolname is easily configured to work with new \mves.
%\info{R3C7, R4C3, R4C6}

The \emph{tick duration} is the amount of time it takes the \mve to complete a single iteration of the game loop,
and \emph{tick distribution} is the percent of tick time the \mve spent simulating each workload component, such as simulating entities.
Both metrics are directly related to game response time and are important indicators of game performance.
More detail about the relationship between these metrics is available in \Cref{sec:model:mve-archi}.

% The Metric Externalizer requires explicit support for the type of \mve tested using \toolname.
% The current implementation of \toolname supports Java-based \mves, and uses a combination of in-game debugging tools and Java Management Extensions~(JMX) to expose these metrics.

% To know what components of the workload contribute most to the tick duration it is necessary to use the internal performance analyzer instrument included in the three Minecraft-like games we test, which \toolname activates through the server console. This instrument logs the percent of tick time spent on given tasks over a period of many ticks, reporting an average value throughout the experimental duration. 

\subsubsection{System-level Metrics}
\label{sec:design:metrics:system}

\toolname captures system-level metrics to allow users to perform a more in-depth performance analysis.
\toolname collects system-level metrics using the System Metrics Collector~(\designref{8}),
which queries the operating system twice per second.

\toolname collects CPU utilization, memory usage, the number of operating-system threads associated with the \mve, disk I/O, and network I/O.
These metrics allow users to analyze causes of high tick duration,
and check for potential performance bottlenecks.

% We capture system metrics on the virtual machine running the Minecraft-like game using a python script with the PSUtil library~\cite{psutil}, at a sampling rate of twice per second. 

\section{\newmetricfull metric}
\label{sec:metric}

In this section we present our novel \newmetricfull metric.
We present a definition, analyze its properties, and compare it to existing metrics.

\subsection{\newmetricfull Definition}
\label{sec:design:metrics:derived}
\label{sec:design:metrics:jitter}
\label{sec:metric:definition}



In the context of online gaming, players prefer stable performance to unstable, but on average faster, performance~\cite{DBLP:journals/cacm/ChenHL06, ries2008empirical, normoyle2014player}. Stability facilitates predictability, allowing players to acclimate to game update delays, up to a point.
% Necessity
Thus, it is beneficial to quantitatively analyze the stability of game performance by analyzing the variability of game cycles, or ticks~(see~\Cref{sec:model:mve-archi}). However, existing measures of variability are insufficient, because they do not capture the order of
ticks, outlier values, the duration of the trace, or a combination of these elements.

We describe here our novel \newmetricfull~(\newmetric), a normalized metric
based on \emph{cycle-to-cycle jitter}~\cite{jitterpll,JitterPhase}. %\info{R1C1, R3C10}
In the context of \mves, we measure cycle-to-cycle jitter as the difference in delay between consecutive ticks~(see~\Cref{sec:model:mve-archi}).
This delay starts to vary when the game becomes overloaded. We compute the \newmetric as the normalized sum of \mve cycle-to-cycle jitter.
%%% INTUITION vvv
The cycle-to-cycle jitter considers only the
difference between two consecutive ticks; reports for this metric include the maximum or moving average value. Novel in this
work, our \newmetric metric sums the differences, and normalizes the result\remove{ing sum by twice the trace duration}.

The full metric equation is shown in Equation~\ref{eqn:jitter}, where
$N_e$ is the expected number of ticks,
$t_i$ is the duration of the~$i^{\text{th}}$ game tick,
$b$ is the delay between ticks when the \mve runs at its intended frequency,
$\max ( b, t_i )$ is the period of tick $i$, and
$N_a$ is the actual number of ticks.

When a tick lasts longer than the $b$ value, the proceeding tick is delayed. Thus, if the game meets its performance requirements $N_a = N_e$, but if it becomes overloaded $N_a \leq N_e$~(i.e., $\exists i : t_i > b \implies N_a \leq N_e$).

%\info{R1.1, R1.3, R3.3c}

\begin{equation}\label{eqn:jitter}
  \text{ISR} = \frac{\sum_{i=1}^{N_a} \left| \max(b, t_i) - \max(b, t_{i-1}) \right| }{N_e \times 2b}
\end{equation}

Using this metric as a measure of variability, the range of possible values is 0 to 1. A \newmetric of 0 indicates no variability:
the tick period is constant for all ticks in the trace.
A \newmetric of 1 indicates maximum variability, and is reached when the sum of differences between consecutive ticks is equal to twice the duration of the trace~(i.e., $N_e \times 2b$).
This value is reached when tick periods alternate between their intended value and extremely large values.
% The first and tick meets the performance requirement (i.e., finishes within $b$ milliseconds), while the second tick has the worst possible performance before the third tick returns to a nominal duration.

\begin{figure}[t]
  \centering
  %   \begin{subfigure}{0.48\linewidth}
  %     \includegraphics[width=\linewidth]{sr-over-scale}
  %     \caption{Behavior of \newmetric for varying outlier magnitudes ($s$).}
  %     \label{fig:metric:sr-over-scale}
  %   \end{subfigure}
  %   \hfill
  \begin{subfigure}{0.48\linewidth}
    \includegraphics[width=\linewidth]{sr_over_period-1}
    \caption{Behavior of \newmetric for varying outlier periods ($\lambda$).}
    \label{fig:metric:sr-over-period}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.48\linewidth}
    \includegraphics[width=\linewidth]{case1-operational-1}
    \caption{Example traces resulting in different \newmetric values.}
    \label{fig:metric:sr-example}
  \end{subfigure}
  \caption{Numerical analysis of \newmetricfull. Higher values indicate higher performance variability. $s$ indicates the outlier scaling factor. $\lambda$ indicates the period between outliers in number of ticks.}
  \label{fig:metric:sr}
  \vcutL{}
\end{figure}


% As a simple metric of overall performance, we use the arithmetic mean of all ticks in the trace.
\subsection{Analysis of \newmetric Behavior}
\label{sec:metric:numanalysis}

We analyze the behavior of \newmetric by modeling a trace where every $\lambda$~ticks, one tick has a duration of $sb$, while the others all have duration $b$. This means 1 in $\lambda$ ticks exceeds the performance requirement by a factor $s$. This allows expressing \newmetric as $\newmetric=\frac{s-1}{s+\lambda-1}$.
A plot of this function and an example trace based on this model are available in Figure~\ref{fig:metric:sr}.

Figure~\ref{fig:metric:sr-over-period} shows how \newmetric responds to outlier scaling and frequency.
The horizontal axis shows~$\lambda$, which is the number of ticks between outliers, and the vertical axis shows the value of \newmetric. The curves show the value of \newmetric for three values of $s$. The three values of s~(2, 10, 20) indicate that all outliers exceed the latency requirement by a factor 2, 10, or 20, respectively.

\emph{The plot shows that \newmetric increases when outliers become larger~(increasing s),
and when outliers are more common~(lower $\delta$).}
For example, a tick exceeding $b$ by a factor 10~($s=10$) every 25 ticks~($\lambda = 25$) results in an ISR value of 0.26.

% Figure~\ref{fig:metric:sr-over-period} shows that \newmetric decreases quickly when the period between outliers increases, but does so more slowly for larger outliers~(e.g., $s = 20$).
% The horizontal axis shows the number of ticks between outliers~($\lambda$), and the vertical axis shows \newmetric.
% When outliers are relatively small (e.g., $s=2$), the maximum value of \newmetric is relatively low ($\frac{1}{3}$), and decreases rapidly when $\lambda$ increases.
% For large outliers ($s=20$), \newmetric values are close to 1 when outliers are frequent ($\lambda$ close to 2), and decreases to reach $0.16$ when $\lambda=100$.

Figure~\ref{fig:metric:sr-example} shows two example traces: High ISR and Low ISR.
Both traces contain 1000 ticks.
The horizontal axis shows time, and the vertical axis shows tick duration.
Most ticks have a duration below 50\,ms (b), but each trace has five outliers with a scaling factor of 20, resulting in a 1\,second spike.
For the Low ISR trace, all outliers are the start of the trace,
whereas in the High ISR trace the outliers are evenly distributed over time.
While the statistical distributions of the traces are identical,
the ISR for the Low ISR trace is 0.009, the ISR for the High ISR trace is 0.15, an order of magnitude higher.

\begin{table}[t]
  \centering
  % \begin{center}
  % \caption{Metrics collected by \toolname. Src is source of the metric, where M is Minecraft-like game server, C is the clients, S is system, and D is derived.}
  \caption{Comparison of \newmetric with existing variability metrics.}
  \label{tab:metric_comp}
  \vcutS{}
  \begin{tabular}{lccc}
    \toprule
    \textbf{Metric}                         & \textbf{Order}     & \textbf{Irregular} & \textbf{Normalized} \\
                                            & \textbf{Dependent} & \textbf{Sampling}  &                     \\
    \midrule
    Standard deviation                      & \xmark             & \xmark             & \xmark              \\
    Allan variance~\cite{riley2008handbook} & \cmark             & \xmark             & \xmark              \\
    Jitter~\cite{schulzrinne2003rfc3550}    & \cmark             & \cmark             & \xmark              \\
    % \midrule
    \textbf{\newmetric}                     & \cmark             & \cmark             & \cmark              \\
    \bottomrule
  \end{tabular}
  % \end{center}
  %\vcutL{}
\end{table}

\subsection{Comparing \newmetric to Alternative Metrics}
\label{sec:metric:compare}

Table~\ref{tab:metric_comp} compares \newmetric to existing measures of variability.
Standard deviation captures spread from an average value. It is not order dependent, and thus is not a measure of stability, but dispersion.

% Allan variance
Allan variance is used in the field of electrical engineering as a time domain measure of frequency stability, typically applied to clocks or oscillators~\cite{riley2008handbook}. Allan variance is order dependent, but relies on a constant sampling frequency and a continuous sampling domain. Neither property is applicable to the duration of tick values.

% Jitter
Jitter is defined in the domain of networking as the smoothed absolute difference between consecutive packets~\cite{schulzrinne2003rfc3550}. While most similar to \newmetric, which is based on cycle-to-cycle jitter, it is not normalized, but rather reported as an average and defined for any packet, rather than an entire sampling duration.






==> TECHNICAL REPORT ICPE2023 Meterstick NEW/content/4_MF_CloudEnv.tex <==

\subsection{\ref{mf:cloud-perf-variability}: \mves exhibit increased variability in commercial cloud environments}
\label{sec:mf3}
\label{sec:experiments:cloud-perf-variability}
\begin{figure}[t]
    \includegraphics[width=\linewidth]{figures/50iter_tick_and_jitter_boxplot.pdf}
    \vcutL{}
    \caption{Distribution of tick times and \newmetric from 50 iterations of the Players workload. Whiskers extend to $\pm$ 1.5 $\times$ IQR, bounded by the minimum and maximum values.} % \das environment pinned to 2 cores.}
    \label{fig:50_iter_jitter}
    \vcutL{}
\end{figure}
In our experiments, all \mves show increased performance variability in terms of both variability (i.e. \newmetric) and tick times, when run on the AWS and Azure cloud environments, compared to the self-hosted \das.
Figure~\ref{fig:50_iter_jitter} shows \newmetric and tick time distribution across 50~iterations of the Player workload~(see \Cref{sec:player_workloads}) of all three games (on the vertical
axis) in \das (green), Azure (blue), and AWS (red).


% that the variance in normalized VI across iterations is greater on cloud environments. It depicts the distribution of normalized VI from 50 iterations of the Players workload, which consists of 25 simulated players using the ``bounded random" behavior (described in \Cref{sec:player_workloads}) for each Minecraft-like game and on each of the DAS5 2-core, AWS, and Azure environments.

% The horizontal axis is variability, the vertical axis is Minecraft-like game, and colors indicate environment (where the DAS5 is pinned to 2 cores). Box plot central line indicate median. 

The results show that all three games are the most stable, with the lowest median \newmetric (line inside boxes) and the lowest \newmetric overall, when run on \das.
The \emph{maximum} \newmetric observed on the \das is 0.021 (Forge), which is smaller than 0.029, the \emph{minimum} \newmetric observed in AWS and Azure~(PaperMC). Distribution of tick time follows a similar trend, with each game exhibiting lowest mean and median tick time on the \das, as well as the smallest interquartile range (IQR).


From this result, we highlight two surprising observations.
First, no game performs best in all environments.
On \das, PaperMC performs best, slightly outperforming Minecraft with a median \newmetric of 0.007 and 0.010 respectively.
Although PaperMC also has the lowest median \newmetric on Azure, it simultaneously has the highest IQR of both \newmetric, 0.028 compared to Forge's 0.009 and Minecraft's 0.011, and tick time, 40.75 to Forge's 23.25 and Minecraft's 26.71.
Moreover, on AWS, PaperMC is the worst performing game, with a median \newmetric of 0.094 and a median tick time of 48.98.
Second, neither cloud performs best for all games.
While AWS performs better for Minecraft and Forge, Azure performs best for PaperMC.


% In both the Azure and AWS commercial cloud environments each Minecraft-like game exhibited increased variation between iterations compared to the DAS5 environment. Of particular interest is PaperMC, as on the DAS5 it operated with the smallest variation in VI between iterations but on has the largest variation of the servers on Azure and AWS. Additionally, it reverses the typical ordering of environments wherein for Minecraft and Forge the AWS environment yields lower variation compared to Azure.

Increased performance variability in commercial cloud environments is a well-documented phenomenon~\cite{variability,tamingvariation,blackboxvariation,storagevariability}, with a wide variety of sources identified for the cause of increased variability, including hardware manufacturing differences, shared tenancy of hardware and networks, specific software configurations, and resource allocation and scheduling systems.
With so many variables operating in the context of commercial cloud hosting, it is infeasible to identify a single source responsible for the variability of these games, especially since commercial cloud hosting companies do not make internal data on resource allocation and shared tenancy publicly available.
However, we can conclude that this variability observably impacts the performance of \mves, and can be compared between \mves and commercial cloud services.


==> TECHNICAL REPORT ICPE2023 Meterstick NEW/content/4_MF_Entity.tex <==
\subsection{\ref{mf:entities-expensive}: Processing entity-state is computationally expensive}\label{sec:mf4}
\label{sec:experiments:entities-expensive}

\begin{figure}[t]
    \includegraphics[width=\linewidth]{figures/tick_percents.pdf}
    \caption{Distribution of tick duration attributed to specific \mve features on AWS environment. ``Other'' is the unspecified category.} % and values less than 1 percent.}
    \label{fig:aws_tick_percents}
\end{figure}

%Having shown that \envworkloads impact performance, we now analyze what workloads components contribute highly to increasing computational complexity.
Entity workload components account for a large majority of computation time and state update messages.

Figure~\ref{fig:aws_tick_percents} shows that entity related workload components contribute to a majority of non-waiting tick computation time. After entities, the next most time intensive component is environment rule processing, and then block creation or destruction. 

The horizontal axis is percentage of tick computation time. The vertical axis on the left is \mve and Workload on the right. The color of each bar indicates workload operation, and the width of each bar corresponds to their share of tick computation time throughout the experimental duration on the AWS environment. 

Entities account for a majority of non-waiting tick time during every workload on each server. Most notably, PaperMC has a much smaller proportion of entity calculation time under each workload compared to Minecraft and Forge. During the TNT workload, in which Minecraft and Forge show large percentages of entity tick computation time compared to both the Control and Farm workload, PaperMC has only a small increase. This reduction in Entity computation may explain how PaperMC manages its comparatively high performance during the TNT workload as seen in \ref{mf:variability-player-experience}.

\begin{table}[t]
  \begin{center}
    \caption{Percentage of network messages sent during experiments on AWS that are related to entities. Computation refers to percentage of messages sent and communication refers to percentage of bytes sent.
    \label{tab:messages}}
    \begin{tabular}{l l r r}
      \hline
      \textbf{Server} & \textbf{Workload} & \textbf{Computation} & \textbf{Communication}\\
      \hline
       & Control & 97.5& 3.8 \\
      Minecraft & Farm  & 91.7& 17.4\\
       & TNT & 97.0& 9.8 \\
       \hline
       & Control  & 97.2& 3.2\\
      Forge & Farm  & 86.7& 9.7\\
       & TNT  & 97.1& 10.3\\
       \hline
       & Control &89.1& 1.3 \\
      PaperMC & Farm  & 47.5& 1.2\\
       & TNT  &94.8& 3.5\\
      \hline
    \end{tabular}
  \end{center}
\end{table}

Table~\ref{tab:messages} shows that entity-related state updates account for a majority of messages sent to the client from the server in all configurations except PaperMC running the Farm workload. Conversely, entity-related state updates account for only a small percent of network bytes sent. 

Thus, we find that efficient computation and dissemination of entity state is a crucial performance challenge to \mves. Unlike environment processing, which exhibits spacial locality; entities require computation and take actions regardless of proximity to players, terrain or other entities. 
%This ability to move freely within the grid world means that physics simulation features such as gravity, liquid dynamics and collision must also be computed each tick for each entity. As \mves have no pre-calculated paths, way-points, or fixed locations, entities must make use of grid-based pathfinding, and their paths must be recalculated upon each terrain state update within their vicinity. Similarly, entities in \mves require computation even before they have been created. As there are no set locations for entities to appear, these must be calculated each tick from the configuration of local game state: terrain, player positions, and existing entities.

==> TECHNICAL REPORT ICPE2023 Meterstick NEW/content/4_MF_Hardware.tex <==
\subsection{\ref{mf:default-hardware-insufficient}: Using recommended hardware results in significant performance variability}
\label{sec:mf5}
\label{sec:experiments:default-hardware-insufficient}

\begin{figure}[t]
    \includegraphics[width=\linewidth]{figures/NodeSize_jitter_and_tick_boxplot.pdf}
    \vcutL{}
    \caption{Tick time distribution and \newmetric during TNT workload on various AWS node sizes. Whiskers extend to $\pm$ 1.5 $\times$ IQR, bounded by the minimum and maximum values. Black diamond indicates arithmetic mean.}
    \label{fig:node_sizes}
    \vcutL{}
\end{figure}

Recommended hardware configurations in cloud environments result in unacceptable levels of performance variability, which degrades player experience.
By using more powerful cloud hardware, performance variability can be limited to acceptable levels.
Figure~\ref{fig:node_sizes} shows this result, showing both the mean tick duration and \newmetric for varying VM sizes in AWS.
% For further analysis, see the technical report~\citeanon{techreport}.
We use the notation \emph{2XL}, \emph{XL}, \emph{L} to denote AWS VM sizes~\emph{t3.large}, \emph{t3.xlarge}, and \emph{t3.2xlarge} respectively.

Companies that specialize in cloud hosting of \mves commonly list recommended hardware configurations, with the most frequent recommendation being 2\,vCPUs and 4\,GB memory.
An overview of these recommendations is available in Table~\ref{tab:hardware_recs}.
These recommended values are significantly lower than those listed on the community-driven Minecraft wiki, which recommends a dedicated full CPU (e.g., Intel i5 or i7, or AMD Ryzen 5 or 7) and 6\,GB memory~\cite{serverrequirements}. This indicates that players experienced performance problems with the recommended hardware configuration.

% Figure~\ref{fig:node_sizes} shows that increasing node size on AWS results in significant decreases in both performance variability and mean tick duration.

Figure~\ref{fig:node_sizes} shows that using the recommended hardware configuration as listed by cloud-hosting companies,
which corresponds to the \emph{L} node type, results in poor performance and significant performance variability.
On this node size, each \mve becomes significantly overloaded by \envworkloads and exhibits high performance variability.

The larger node types \emph{XL} and \emph{2XL} have 4 and 8 vCPUs respectively~\cite{amazont3}.
While \emph{XL} provides better performance and less performance variability than \emph{L}, it remains insufficient to keep the mean tick time below 50\,ms.
The \emph{2XL} node type is required to provide sufficiently low mean tick duration.
However, this node type still shows significant performance variability for Minecraft (green cross) and Forge (blue square),
which means these games can still become overloaded temporarily, as shown in \Cref{sec:experiments:envworkloads-perf-variability}.

% The top subplot vertical axis is variability expressed as normalized jitter, and the bottom subplot is mean tick duration in milliseconds, where the black dashed line is the overloaded threshold of 50ms. Marker color indicates Minecraft-like game.

% We find that the t3.large node size, which is most similar to the recommended configuration, is insufficient for maintaining quality of service of the Minecraft-like games tested.  Additionally, we observe that larger node sizes reduce both performance variability and mean tick duration, such that the t3.2xlarge size yields acceptable levels of each for all Minecraft-like games tested.

Interestingly, we observe that the benefit of more powerful hardware varies per \mve.
Specifically, while PaperMC's (red circle) performance instability (i.e., \newmetric) increases significantly when decreasing hardware resources, from 0.025 to 0.08 in the top-right sub-plot, it is the only game whose mean and 75th percentile tick duration stays well below the 50\,ms threshold.
Further analysis shows that, while PaperMC becomes overloaded and its tick duration exceeds 50\,ms, the number of extreme outliers is low, preventing this performance problem from becoming visible in the mean tick duration.


==> TECHNICAL REPORT ICPE2023 Meterstick NEW/content/4_MF_Latency.tex <==
\subsection{\ref{mf:variability-player-experience}: Performance variability can make \mves unplayable}\label{sec:mf1}
\label{sec:experiments:variability-player-experience}


% Performance variability on AWS causes game response time vary, to the extent that the Minecraft-like games tested had noticeable up to unplayable amounts of input latency.

Due to significant performance variability, the median and mean game response times give an optimistic view of game
performance, and is worse than the performance observed by players.
Figure~\ref{fig:aws_response_time} depicts the result, and shows that the 95th percentile of game response time can be up to 4.1 times higher than the arithmetic mean, and exceed by more than a factor of~12.8 the threshold that makes the game unplayable.
In real-time games, a temporary spike in delay can significantly affect the user's experience, similar to a temporary freeze in a phone call or video stream.

% Figure~\ref{fig:aws_response_time} shows the server response time for player actions, showing that increased performance variability as a result of \envworkloads in the AWS environment causes average response time to increase, with some \envworkloads causing response times that greatly exceed both the noticeable and unplayable input latency times of 60ms and 118ms, respectively~\cite{latency60ms,unplayable118ms}. PaperMC is omitted as it uses a dedicated asynchronous thread for chat messages, separately from the game tick.
\begin{figure}[t]
    \includegraphics[width=\linewidth]{figures/rtt_boxplot.pdf}
    \vcutL{}
    %\vspace*{-0.35cm}
    \caption{Game response time in AWS environment when running separate \envworkloads.
        %Horizontal axis split into two sections (0-210 and 211-1550) that scale linearly. 
        Whiskers indicate 5th and 95th percentile respectively.
        The black diamonds indicate arithmetic mean.}
    \label{fig:aws_response_time}
\end{figure}
Figure~\ref{fig:aws_response_time} shows the response time (horizontal axis)
for two \mves (Minecraft in green, and Forge in blue) under three different workloads (vertical axis).
The workloads and response time metric are described in \Cref{sec:design:workloads} and \Cref{sec:design:metrics:application} respectively.
PaperMC is omitted as it uses a dedicated asynchronous thread for chat messages, separately from the game tick.
The whiskers extend to the 5th and 9th percentiles, respectively,

and the black diamond indicates the arithmetic mean.
The \emph{Noticeable Delay} line~(at~60\,ms, in orange) and \emph{Unplayable Game} line~(at~118\,ms, in red) indicate high game-latency which respectively marks the values where latency becomes noticeable to players and makes the game so unresponsive it becomes unplayable~\cite{latency60ms,unplayable118ms}.

% The horizontal axis is game response time, which measures how long the game server takes to resolve a player action and send the result. This axis is split into two sections from 0-200 ms and 201-1550 ms that each scale linearly. Extreme maximum values are indicated with an arrow. The noticeable and unplayable input latency thresholds are shown with vertical lines of orange and red respectively.

% The vertical axis is the Minecraft-like game under test and the workload it is running, where color indicates the game and the label on the left is the workload. The colored section around the box plot indicates the distribution of values. The black dashed line indicated arithmetic mean and the central line in the box plot indicates median.

Under the Control workload~(top two boxes), the 95th percentile is below the noticeable threshold for both Minecraft and Forge.
% I think we keep this specific maximum as it explains the outliers
However, the maximum value for Forge~(514\,ms) is 20.7~times larger than the mean, and the maximum value for Minecraft~(679\,ms) is exceeds by 7.4~times the Unplayable threshold at 118\,ms.
These outliers occur directly after a player connects to the game.
This means that, even with good average performance, the game can still be unplayable if players frequently connect, which is a common occurrence in online multiplayer games.
% We conjecture this delay is caused by the game serializing and sending large amounts of terrain data to the new player.

Compared to the Control workload, the Farm and TNT workloads show significantly more performance variability, pointing to a further degradation of player experience.
\emph{In all cases, the mean and median values give an overly optimistic view of the game's performance.}
For the Farm workload, the mean and median values for Forge~(third bar from the top) indicate the response time is noticeable, but not unplayable. However, the plot shows a 95th percentile of 225.8\,ms, which is 1.9 times as high as the Unplayable threshold.
For Minecraft~(fourth bar from the top), the mean and median values indicate that the response time is not noticeable for players.
However, the plot shows that performance variability causes the response time to exceed the Noticeable threshold more than 25\% of the time~(box's right edge exceeds the Noticeable threshold), and exceeds the Unplayable threshold more than 5\% of the time.
% With non-trivial \envworkloads the duration of response time increases.
% For instance, 
% the Farm workload causes more than 50\%  of input latencies to be noticeable for the Forge server. For the Minecraft server the effect is less pronounced but still causes >25\% to be noticeable.
The TNT workload causes the highest performance variability for both Forge and Minecraft (bottom two boxes, 547\,ms interquartile range for Forge and 503\,ms for Minecraft).
In both cases, the median response time is below the noticeable threshold, while the
95th percentiles are 12.7 times the unplayable threshold, and the maximum observed values (indicated with black arrows) are at least 19 times larger than the unplayable threshold.

% The TNT \envworkload caused both the most variation ) and highest average (370.4ms for Forge, 316.2ms for Minecraft) of response time, with latency values up to an order of magnitude higher than the unplayable threshold. 

From results in this section, we conclude that the mean and median values give an overly optimistic view of \mve performance, and that performance variability in \mves results in noticeable and unplayable game latency,
impacting players.
%negatively affecting players.

% In Minecraft-like games, the frequency of state updates that players receive is directly related to the time it takes the server to complete iterations of the tick loop. If there is significant performance variability, there is also variation in state updates. From the point of view of the players, this results in variation in response time for player actions. If a high percentage of player actions have noticeable, or even unplayable latency, the Minecraft-like game as a whole fails to provide quality of service. As we observe significant variation in input latency to the extent of reducing player experience to an unplayable state, we conclude that this performance variability negatively affects players. 


==> TECHNICAL REPORT ICPE2023 Meterstick NEW/content/4_MF_PAWs.tex <==

\begin{figure}[t]
    \includegraphics[width=\linewidth]{figures/PAWs_jitter_scatter_all.pdf}
    \vcutL{}
    \caption{\newmetric for each \mve on the AWS and \das environments. The Lag workload crashed all \mves on AWS; see text for explanation.
        \Cref{sec:player_workloads} defines the ``Players'' workload.}
    \label{fig:paw_jitter_scatter}
    \vcutM{}
\end{figure}

\subsection{\ref{mf:envworkloads-perf-variability}: \Envworkloads cause significant performance variability}\label{sec:mf2}
\label{sec:experiments:envworkloads-perf-variability}

\begin{figure}[t]
    \includegraphics[width=\linewidth]{figures/aws_tick_line.pdf}
    \vcutL{}
    \caption{Tick time over time for each \mve in the AWS environments running the Control, Farm, TNT and Players workloads. The Lag workload on AWS is omitted as each \mve crashes. \Cref{sec:player_workloads} defines the ``Players'' workload.}
    \label{fig:paw_tick_line}
\end{figure}

\Envworkloads cause significantly increased performance variability on each game and in each environment tested,
and can overload or crash the game.
Figure~\ref{fig:paw_jitter_scatter} shows the performance variability of each \mve when running \envworkloads on AWS and \das.
Compared to the control workload, each \mve on each environment exhibits higher performance variability when operating \envworkloads.

Figure~\ref{fig:paw_jitter_scatter} shows performance variability, quantified using \newmetric (see Equation~\ref{eqn:jitter}).
The three top-level rows show three environment configurations, each containing five workloads.
The color and shape of the marker indicate one of three \mves.

% Here 0 indicates no variability (every tick less than 51ms) and 1 indicates that each consecutive tick fluctuated from an overloaded to non-overloaded state. The vertical axis shows environment and workload, and the color of marker indicates the Minecraft-like game. Aside from \envworkloads, the \textit{Players} workload (n=25) is shown as a comparison. The Lag workload on AWS is omitted as each Minecraft-like game would crash upon loading the workload. 

\Envworkloads (i.e., Farm, TNT, Lag) cause significantly higher performance variability than the player workload and control workload for all games in all environments, with the exception of PaperMC on AWS (red circles in the top row).
This provides evidence that \envworkloads cause significant performance variability.
Further analysis into the behavior of PaperMC reveals that it contains performance optimizations specifically for handling TNT explosions, improving its performance on the TNT workload, and Redstone, a simulated block type which is used in the Farm workload (analysis of PaperMC given in ).
%technical report~\citeanon{techreport}).
This provides evidence that the performance variability caused by these \envworkloads are known to the \mve community and can (at least partially) be addressed through engineering.

% In all three environment configurations, all three games show increased performance variability when running the Farm and TNT workloads, compared to the Control workload.
% Under most environment workloads, PaperMC tends to be the least variable of the three games tested.
% Notably, even on the \das environment with 16~cores, the Farm, TNT, and Lag workloads cause substantial increases in variability, whereas the Player workload is comparable to the Control workload. 

Of all workloads, the Lag workload causes the most performance variability.
Further analysis reveals that this happens because this workload consists mainly of parts which are only simulated every other tick, causing the game to alternate between extremely short and extremely long ticks.
This maximizes the value of \newmetric, which is based on the difference in duration between consecutive ticks.
% Further analysis of this result reveals that this is caused by the Lag workload significantly extending the duration of every other tick, resulting in a near-maximum VI.
There are no results for running the Lag workload on AWS because all three \mves crash when a player joins and the environment simulation begins. The corresponding increase in tick duration causes the player's connection to time-out, forcing each \mve to stop. %and the \mve forcibly stops when it cannot write player data to file.

% The Lag workload results in a worst-case scenario: it causes all games tested to crash on the AWS environment, and a near maximal amount of performance variability in the DAS5 environment.

Figure~\ref{fig:paw_tick_line} shows the game's tick duration over time for each game when running on AWS. The dashed black line indicates the overloaded threshold at 50\,ms,
and the green line allows calibrating the vertical axis across the four sub-plots.

% Figure~\ref{fig:paw_tick_line} depicts the tick duration over time from each server tested on both the DAS5 and AWS environments, with a black dashed line depicting the overloaded point at 50ms. It shows that in both environments the performance variability associated with player agnostic workloads can strongly affect the performance of each game, such that \envworkloads workloads alone can overload or even crash the Minecraft-like games tested. 

% Each subplot depicts time on the horizontal axis and tick duration on the vertical axis, with line colors indicating Minecraft-like game. Subplot column indicates workload and row specifies environment. The Player workload is shown (farthest right column) with an orange background.

%\begin{figure*}[t]
%    \includegraphics[width=\textwidth]{figures/PAWs_tick_line_al%l.pdf}
%    \caption{Tick time over time for each server in the DAS5 and %AWS environments running the Control, Farm, TNT and Lag %workloads. The Lag workload on AWS is omitted as each server %would crash before simulated players could join. As a comparison %the Control workload with 25 moving players is shown in orange.}
%    \label{fig:paw_tick_line}
%\end{figure*}

The stability observed when running the Control workload in Figure~\ref{fig:paw_jitter_scatter} is visible in the top-left sub-plot in Figure~\ref{fig:paw_tick_line} as three relatively stable curves with few spikes.
In contrast, the high performance variability observed for the Farm and TNT workloads is visible in the top-right and bottom-left sub-plots as jittery curves.
The Farm workload depicted in the top-right shows curves which change value at high frequency, resulting in high \newmetric.
% We hypothesize this is because the farm workload causes different amounts and types of objects to be simulated each tick.
PaperMC's tick durations are frequently below the 50\,ms threshold, resulting in lower \newmetric.
The TNT workload depicted in the bottom-left shows curves which change value at a much lower frequency, but reach significantly higher values, exceeding 2500\,ms for both Minecraft and Forge.
Similar to the Farm workload, PaperMC's tick durations are often below 50\,ms, resulting in lower \newmetric.

% stable and operates with a majority of tick duration under the overloaded threshold, though the Forge server on AWS briefly spikes to overloaded durations. 
% The Farm workload, compared to the Control, causes increases in both mean tick duration and variation for all games on each environment. The Farm workload's increased performance complexity corresponds to the operation of in-game simulated construct resource farms (see \Cref{sec:Workloads} and \ref{sec:environment_workloads}). On the AWS, the tick durations of both the Minecraft and Forge servers are above the overloaded point throughout the experimental duration, with noisy spikes up to the 100ms to 200ms range for Minecraft, and 200ms to 300ms for Forge. PaperMC on AWS performs slightly better, with a baseline tick duration just under the overloaded point and pulses causing increases to the 50ms to 200ms range.

% The TNT workload shows comparable performance to the control workload on each environment until the 20 second mark, when the TNT voxels activate and cause a large chain reaction (see \Cref{sec:environment_workloads}). This causes all three servers to become overloaded on both AWS and the DAS5. On AWS, the Forge and Minecraft servers have single tick durations peaking at around 2.5 and 3 seconds respectively, more than 500 times the overloaded threshold. Neither server returns to an nominal tick duration before the end of the experimental duration. Notably, the PaperMC server is not nearly as effected. It peaks at a tick duration of 425ms and returns to a sub-overloaded times in less than 10 seconds. 
% The TNT workload on the DAS5 2 and 16 core environments results in comparable trends, though with each server reaching maximum tick durations that are shorter than on AWS, and returning to nominal tick duration in less time.

% On the DAS5, the Lag workload causes each server to alternate between long and short ticks, due to the lag machine simulated construct which is specifically designed to cause a high volume of environment state updates every other tick. The duration of the longer ticks on the 16 core environment is around 6 seconds for Minecraft and Forge, and around 2 seconds for PaperMC. On the 2 core environment Minecraft specifically has even higher tick peaks, up to 12.9 second durations for single ticks. Tick duration of this magnitude reduces game update frequency from the nominal 20Hz to .17Hz, effectively freezing the game from the perspective of the players. On AWS, the performance impact of the Lag workload is enough to cause each server to crash.



==> TECHNICAL REPORT ICPE2023 Meterstick NEW/content/4_experimental_analysis.tex <==

\section{Real-World Experiments}\label{sec:experiments}

To address contribution~\ref{contrib:experiments}, we present here the setup and results from our real-world experiments.
We use \toolname to evaluate the performance variability of three \mves: Minecraft, Forge, and PaperMC. Our experiments use the workloads described in \Cref{sec:design:workloads}, and are conducted on two commercial cloud environments, Amazon~AWS and Microsoft~Azure, as well as on DAS-5, a supercomputer for scientific workloads~\cite{das5}. 

%including choice of Minecraft-like games and hardware, then provide an overview of findings from our experiments as well as detailed analysis of each finding.

% \subsection{Main Findings}
\label{sec:main_findings}
% In this section we present and analyze the data collected using the \toolname benchmark while running the Minecraft, Forge and PaperMC servers with the workloads listed in \Cref{sec:benchmark_workloads} on the DAS5, AWS and Azure environments. Our main findings are:
\begin{enumerate}[label=\textbf{MF\arabic*}]
  \item\label{mf:variability-player-experience} Performance variability can make
        \mves unplayable~(\Cref{sec:mf1}).
        We find that the maximum response time can be up to 20.7 times higher than the arithmetic mean, and exceed by more than a factor of~7.4 the threshold for playable games.

  \item\label{mf:envworkloads-perf-variability} \Envworkloads cause significant performance variability~(\Cref{sec:mf2}).
        We find that \envworkloads introduce significant performance variability, increasing \newmetric by 0.04 up to 0.92. This variability can overload popular \mves by 58 times the normal tick duration and even crash the game.

        % in both average and best-case environments can overload popular \mves by up to 270 times the nominal tick duration in extreme cases.

  \item\label{mf:cloud-perf-variability}  \mves exhibit increased variability in commercial cloud environments compared to self-hosted environments~(\Cref{sec:mf3}).
        We show that both clouds, AWS and Azure, introduce additional performance variability between iterations of the same workload compared to the local environment, \das. The choice of cloud causes a 1.39 up to 15.44 times increase in \newmetric IQR and a 1.09 up to 5.61 times increase tick time IQR. The minimum observed \newmetric for both clouds exceeding the maximum observed \newmetric on \das.

  \item\label{mf:entities-expensive} Processing the state of entities is computationally expensive~(\Cref{sec:mf4}). Entity-related computations account for a majority of the non-idle tick distribution in all experiments.

  \item\label{mf:default-hardware-insufficient} The common hardware resource recommendations are insufficient to avoid performance variability~(\Cref{sec:mf5}).
        The recommended node size exhibits high performance variability and high mean tick duration.
        Larger node sizes result in lower values of both, such that a node with 8~vCPUs reduces performance variability and mean tick duration to acceptable levels.

        % \item\label{mf:entities-expensive} Processing the state of entities is computationally expensive~(\Cref{sec:mf4}).

\end{enumerate}

\subsection{Experimental Setup}\label{sec:experimental_setup}

In this section we describe our experimental setup.
In our experiments, we evaluate three \mves, i.e., the systems under test, in three different environments.

% We run experiments using the \toolname benchmark on three environments and measure the performance variability of three Minecraft-like games.
% The environments selected are AWS, Azure and self-hosted on the DAS5 cluser, where the hardware configuration of each environment (2vCPU, 8GB RAM) was chosen based on our survey of recommended hardware from companies that offer Minecraft-like game hosting. The Minecraft-like games selected are Minecraft, Forge and PaperMC.

\subsubsection{System under test}

We use in our experiments three \mves that use the Minecraft protocol: the original Minecraft as developed by Mojang~\cite{mcserver}, \textit{Forge},
% which is popular with mod makers,
and \textit{PaperMC}.
% which the authors claim is engineered for high performance.
We select these services because of their popularity and utility.

We choose the official Minecraft server~\cite{mcserver}, as it is the default service that most users and hosts operating Minecraft servers employ. This includes users of the server hosting service \textit{Realms}, which is advertised inside the Minecraft client~\cite{Realms}. Notably, the Minecraft service does not allow for gameplay modifications~(``\textit{mods}") of any kind.

% The second is 
% Forge which extends the Minecraft protocol with an API supporting community-made mods.
\emph{Forge} is the most popular \mve for operating modified (i.e., \emph{modded}) services~\cite{forge}. Of the top-50 most downloaded Minecraft mods,
45~work exclusively with Forge.
Of the 5~mods that are not exclusive to Forge, only one is incompatible with it~\cite{mcmods}.
% only~5 are not exclusive to the Forge API, and of those~5, only~1 is not available on Forge~\cite{mcmods}.
\emph{PaperMC} is marketed as a high-performance alternative to Minecraft~\cite{papermc}.
% PaperMC does not support mods, but it does support server-side \textit{``plugins"} that modify the functioning of the game without changing the Minecraft protocol.
While the PaperMC project does not quantify its performance improvement over Minecraft, it does provide documentation of its optimizations, which include extensive changes to threading models and virtual environment processing.

\subsubsection{Deployment Environment}

\begin{table}[t]
  \begin{center}
    \caption{Hardware recommendations from companies that offer cloud hosting of Minecraft-like games. Field marked NP are information not provided to consumers, fields marked V are variable. \label{tab:hardware_recs}}
    \begin{tabular}{l c c c}
      \hline
      \textbf{Service} & \textbf{RAM [GB]} & \textbf{vCPU[\#]} & \textbf{CPU Speed[GHz]} \\
      \hline
      \href{https://www.hostinger.com/minecraft-server-hosting}{Hostinger}~\cite{hostinger} & 3 & 3 & NP \\
      \href{https://server.pro/}{Server.pro}~\cite{server.pro} & 4 & 2 & 2.4 \\
      \href{https://www.skynode.pro/}{Skynode}~\cite{skynode} & 4 & 2 & 3.6\\
      \href{https://scalacube.com/hosting/server/minecraft/plans/public?}{ScalaCube}~\cite{scalacube} & 3 & 2 & 3.4 \\
        
      \href{https://nodecraft.com/}{Nodecraft}~\cite{nodecraft} & 4 & NP & 3.8\\
      \href{https://apexminecrafthosting.com/}{Apex Hosting}~\cite{apex} & 4 & NP & 3.9\\
      \href{https://ggservers.com/}{GGServers}~\cite{ggservers} & 4 & NP & 3.2\\
      \href{https://www.bisecthosting.com/}{BisectHosting}~\cite{bisect} & 4 & NP & 3.4\\
      \href{https://shockbyte.com/}{Shockbyte}~\cite{shockbyte} & 4 & NP & 4.0\\
      \href{https://cubedhost.com/}{CubedHost}~\cite{cubedhost} & 2.5 & NP & 4.5\\
      \href{https://serverminer.com/buy-minecraft-server}{ServerMiner}~\cite{server} & 3 & NP & 4.0\\
      \href{https://www.akliz.net/pricing}{Akliz}~\cite{akliz} & 4 & NP & 3.4\\
      \href{https://ramshard.com/hosting/minecraft}{RamShard}~\cite{ramshard} & 2 & NP & 4.0\\
    \href{https://mcprohosting.com/}{MCProHosting}~\cite{mcpro} & 2 & NP & NP\\
      \href{https://www.gtxgaming.co.uk/}{GTXGaming}~\cite{gtxgaming} & 3 & NP &3.8 \\
    \href{https://stickypiston.co}{StickyPiston}~\cite{stickypiston} & 2.5 & NP & NP\\
      \href{https://hosthavoc.com/minecraft}{HostHavoc}~\cite{hosthavoc} & 4 & NP &4\\
    \href{https://feroxhosting.nl/}{Ferox Hosting}~\cite{ferox} & 4 & NP &NP\\
      \href{https://aquatis.host/minecraft-hosting/}{Aquatis}~\cite{aquatis} & 4 & NP & 4.2\\
      \href{https://pebblehost.com}{PebbleHost}~\cite{pebble} & 3 & NP & 3.7\\
      \href{https://www.meloncube.net/}{MelonCube}~\cite{meloncube} & 4 & NP & 3.4\\
      \hline
      \href{https://docs.microsoft.com/en-us/gaming/azure/reference-architectures/multiplayer-basic-game-server-hosting}{Azure}~\cite{azureserver} &  4 & 2 & V\\
      \href{https://web.archive.org/web/20201126074839/https://aws.amazon.com/getting-started/hands-on/run-your-own-minecraft-server/}{AWS}~\cite{amazonserver} & 1 & 1 & V\\
      \hline
    \end{tabular}
  \end{center}
\end{table}

We evaluate the \mves in two commercial cloud environments, Amazon~AWS and Microsoft~Azure,
and \das, a supercomputer for academic and educational use~\cite{das5}.
We choose AWS and Azure because they are the two cloud environments with the biggest market share, with 32\% and 20\% respectively~\cite{cloudproviders}.
We use \das to evaluate how commercial cloud environments affect the performance variability of \mves, compared to self-hosting these games on dedicated hardware.
% Additionally, to provide a controlled environment baseline to compare against, we run experiments on the \das, a distributed super-computer for academic and educational use~\cite{das5}.

% Commercial cloud providers are incentivized to minimize the total utilization of hardware resources to reduce cost and support more concurrent customers, and to maximize performance-to-price ratios in order to stay competitive in a low-entry market. Typically, this is accomplished through advanced load-balancing systems at a datacenter-wide, per-virtual machine scale. However, to allocate resources at a less granular scale, it is necessary to establish in advance an estimate of hardware usage with a given customer either explicitly, such as through choice of virtual machine size, or implicitly, such as through server `plans' that offer varying levels of service quality. To avoid users overestimating their usage and causing over-allocation of resources, it is common practice to publish recommendations on plans or node sizing for specific tasks.



Our experiments on cloud environments use \emph{T3.Large} and \emph{Standard\_D2\_v3} nodes respectively.
Both node types are equipped with 2\,vCPUs and 8\,GB memory. We choose these nodes based on the default hardware configurations recommended by Minecraft service providers as well as guidelines published by AWS and Azure~\cite{azureserver,amazonserver}.

%For an overview of these hardware recommendations, see our technical report~\citeanon{techreport}.

On \das, we use a regular node, which is equipped with a dual 8-core 2.4\,GHz processor and 64\,GB memory, and limit the number of CPU cores available to the \mve by setting its CPU affinity to two cores, unless indicated otherwise.
Because the \mves used in our experiments run on the Java Virtual Machine (JVM), we limit memory available to the \mve in both cloud an \das nodes by setting the JVM's maximum heap size to 4\,GB.

Table~\ref{tab:hardware_recs} lists a sampling of hardware recommendations from commercial cloud companies that offer Minecraft-like game hosting. If no plan was marked ``recommended," data is taken from plans that are comparable to recommended plan on other services. From these recommendations we find that~2\,vCPU and~4\,GB RAM is the most common configuration. On AWS and Azure it is possible to select specific configurations of hardware, however, to ensure that the Benchmark metric tools have sufficient memory during the experimental duration, we use nodes with at least~8\,GB RAM and limit the heap memory of the Minecraft-like game to~4\,GB using the \texttt{-Xmx} JVM argument in all experiments.


% On AWS we use a ``T3.Large" node, which offers two vCPUs and 8\,GB RAM~\cite{amazont3}. On Azure we use a ``Standard\_D2\_v3" node, which also provides two vCPUs and 8\,GB RAM~\cite{azured3}. Nodes were selected within the same subnet to reduce variation caused by network delay (except for the experiments where this was measured). 

% The \das nodes used each have 16 cores and 64\,GB RAM. Where indicated, CPU core affinity is used to limit the operation of the Minecraft-like server to 2 cores.

\input{content/4_MF_Latency}
\input{content/4_MF_PAWs}
\input{content/4_MF_CloudEnv}
\input{content/4_MF_Entity}
\input{content/4_MF_Hardware}


==> TECHNICAL REPORT ICPE2023 Meterstick NEW/content/5_discussion.tex <==
\section{Actionable Insights and Limitations}
\label{sec:actionable_insights}

The main findings in~\Cref{sec:experiments} lead to \textit{actionable insights}:

%In this section we provide a summary of actionable insights based on our main findings.

% Findings:
% 1. Perf. var. bad
% 2. workloadenv inc. perf. var.
% 3. cloud env. inc. perf. var
% 4. recomm. hardware not enough.
\begin{myitemize}[label=\textbf{I\arabic*}]
    \item\label{ai:reportvariability} Game developers and hardware producers should report performance variability when evaluating the performance of online games, using measures of variance such as \newmetricfull~(see \Cref{sec:metrics}) and the distribution of game response time and \fps. Games must provide consistently good performance to their users. Our experiments show that \mves can be overloaded and become unplayable, even when mean and median performance values indicate good performance~(\ref{mf:variability-player-experience}, Figure~\ref{fig:aws_response_time}).

    \item\label{ai:envworkloads} Game developers and hardware producers should include environment based workloads in their benchmarks for \mves. It is not sufficient to evaluate the performance of \mves using only large numbers of players (i.e., player-based workloads).
    \Envworkloads cause significant performance variability in \mves and make them unplayable~(\ref{mf:envworkloads-perf-variability}, Figure~\ref{fig:paw_jitter_scatter}), and must therefore be included in \mve benchmarks.

    % \item\label{ai:benchmarkvariability} Game developers, hardware producers, and researchers should include \envworkloads in the benchmarking of \mves, and should report performance variability. Environment workloads cause increased performance variability in \mves~(\ref{mf:envworkloads-perf-variability}, Figure~\ref{fig:paw_jitter_scatter}). Increased performance variability causes a corresponding increase in game response time variability, such that the \mves can become unplayable~(\ref{mf:variability-player-experience}, Figure~\ref{fig:aws_response_time}). Thus, game developers, hardware producers, and researchers specializing in human-computer interaction should include \envworkloads in the benchmarking of MVEs. Additionally, they should not only report central measures such as average FLOPS or FPS. These metrics have only limited relevance in the context of \mves. Instead, measures of variance such as normalized jitter~(see \Cref{sec:metrics}) and the distribution of game response time should be reported.

    \item\label{ai:bestcloud} Players should choose their cloud environment depending on their \mve, and should consider self-hosting their game. Our results indicate that choice of best cloud provider depends on the \mve. Minecraft and Forge obtain lower performance variability on AWS,
    while PaperMC obtains lower performance variability on Azure~(\ref{mf:cloud-perf-variability}, Figure~\ref{fig:50_iter_jitter}). Moreover, self-hosting remains a valuable alternative, resulting in significantly lower performance variability overall.

    % 4. recomm. hardware not enough.
    \item\label{ai:hardwarereqs} \mve service providers should increase their hardware recommendations.  Prior work has shown that when asked to estimate in advance the hardware requirements of a given program, users either pick a provided default configuration, or overestimate to an extreme value to avoid performance issues~\cite{userestimatesinaccurate,userestimatessp2,userestimateshpc}. We find that recommended hardware configurations for hosting \mves on cloud environments are insufficient~(\ref{mf:default-hardware-insufficient}) and conclude that users who employ the first strategy will experience decreased quality of service which may cause them to switch to a competing commercial cloud provider. 

    To prevent this, commercial cloud providers should update hardware recommendations in line with our findings in Figure~\ref{fig:node_sizes}: a 2-core size is insufficient, and a node with 8~cores is necessary for smooth operation. The 4-core size provides a balance of cost and performance. Beyond these recommendations, commercial cloud providers should use our benchmark to determine adequate hardware allocations capable of fulfilling the service requirements of \mves under realistic workloads, and further adapt resource scheduling to be aware of the performance patterns of \mves. 

    Similarly, users who seek to avoid adverse performance variability when operating \mve cloud environments
    should choose node sizes comparable to the 8~core t3.2xlarge node, or use our benchmark to compare both various cloud
    providers and the specific \mve implementations.

    \item\label{ai:engineering} Game developers should engineer \mves to reduce impact of \envworkloads.
    Engineering for this goal can reduce the impact (i.e., performance variability) of environment-based workloads by 60\% on the same hardware, as shown by PaperMC operating the Farm workload on AWS~(Figure~\ref{fig:paw_jitter_scatter}).
    The goal of the PaperMC project is to implement a high performance \mve, including efficient processing of \envworkloads.
    We provide an analysis of PaperMC in Appendix~\ref{sec:appendix_a}.
    Developers creating \mves should consider and mitigate the impact of \envworkloads, and use our benchmark to measure, analyze and subsequently reduce the performance variability caused by such workloads. 

\end{myitemize}

% \subsection{Threats to Validity}

% Minecraft-like games, though popular, have only limited publicly available data for relevant variables such as average player count, typical player behaviors, or specific \envworkloads. For such decisions, we have assigned a best-guess value or used a domain coverage approach guided by community and official sources.

% Additionally, though \toolname measures multiple quantitative metrics at both an application and systems levels as well as a quantitative approximation of subjective experience through response time, we have no measurements of subjective values such as player experience. Thus, though we do observe values of server performance becoming both overloaded and highly variable, we cannot conclude to what degree this effects player experience.

%\todoall{Discuss variability metric. We don't know yet how a numerical value corresponds to player experience, except that higher is generally worse. There could also be other metrics.}

%  identify only those limitations that had the greatest potential impact on: (a) the quality of your findings; and (b) your ability to effectively answer your research questions and/or hypotheses.

% env: 
% \begin{foo}
% bar
% \end{foo}
% :-)

\begin{addtext}
    Here we discuss limitations of our work % introduced in \Cref{sec:system-design},
    related to the \newmetricfull metric and the workloads.
    \newmetric cannot be used as a singular performance metric, but rather is designed as an additional axis by which to quantitatively appraise the performance of a game server, by capturing behavior that other metrics cannot. Because \newmetric is a measure of variability over an entire sampling duration, it does not capture extremely poor but stable performance, or the occurrence of singular relatively small outliers. Thus, other measures, such as percentiles, are necessary to observe the magnitude of tick durations and detect lone outliers. It is not currently understood how \newmetric directly relates to player-perceived quality of experience and quality of experience, and should be explored in future work, for instance through player studies.

    The workloads included in \toolname are intended to cover a wide range of realistic \envworkloads, from common to extreme cases. However, there is no publicly available analysis of \envworkload prevalence. Thus, we select \envworkloads
    using proxy metrics such as total views and downloads in online \mve communities,
    % from our knowledge and observation of online \mve communities,
    which may not be representative of all \mve players. Additionally, our experiments measuring the impact of \envworkloads utilized a purposefully minimal player-based workload component.
    Finally, because our experiments focused on \envworkloads, our
    % Our experiment using non-minimal
    player-based workloads (``Players") uses random avatar movement.
    Although real player behavior is likely more complex, no player-behavior models exists for \mves.
\end{addtext}

==> TECHNICAL REPORT ICPE2023 Meterstick NEW/content/6_related_work.tex <==
\section{Related Work}
\label{sec:relwork}
\label{sec:related-work}

We summarize in this section a developing overview of related work.
Overall, this study is the first to evaluate performance variability in \mves.
This is challenging because there is neither a generally accepted set of relevant workloads for \mves,
nor a standardized metric to quantify performance variability in computer systems.

% Perf eval
Closest to our work, Yardstick is an \mve benchmark used to show the limited scalability of \mves~\cite{yardstick}.
The authors use Yardstick to evaluate the scalability and network characteristics of several \mve services.
However, Yardstick does not quantify performance variability, resulting in optimistic results.
Moreover, the authors do not evaluate \mve performance under \envworkloads or in the cloud. %or when deployed in a commercial cloud environment.

The MineRL competition~\cite{DBLP:journals/corr/abs-1907-13440} provides a dataset of Minecraft player
recordings. This dataset provides demonstrations to train artificial intelligence systems to complete a challenging
in-game task. In contrast,
the workloads used in this work focus on commonly observed patterns in the \mve community.
%\info{R4C2}

% Perf MVE
There exist several systems that aim to improve the scalability of \mves.
Manycraft~\cite{DBLP:conf/netgames/DiaconuKV13} increases the maximum number of players in a Minecraft instance by using Kiwano.
Kiwano~\cite{DBLP:conf/ieeehpcs/DiaconuK13} allows horizontal scaling of virtual environments through Voronoi partitioning, but requires a \emph{static environment}, which disables the \mve's modifiable world and is incompatible with \envworkloads.
Similar in many ways to Manycraft, Koekepan~\cite{DBLP:conf/netgames/EngelbrechtS13} uses zone-partitioning and scales horizontally.
Dyconits~\cite{DBLP:conf/icdcs/DonkervlietCI21} are a distributed architecture that scales \mves vertically, through the use of dynamically managed consistency-units. 
None of these approaches considers explicitly performance variability.

% Koekepan~\cite{DBLP:conf/netgames/EngelbrechtS13} is \replace{another}{a} distributed architecture for Minecraft. Similar to Manycraft, Koekepan uses zone-partitioning and scales horizontally. Dyconits~\cite{DBLP:conf/icdcs/DonkervlietCI21} are a distributed architecture 
% %by partitioning the world into zones. Koekepan supports a modifiable environment, but currently lacks a performance evaluation. 

% Perf variability
Iosup et al.~\cite{DBLP:conf/ccgrid/IosupYE11} find that commercial cloud environments exhibit significant yearly and daily performance variability patterns.
The authors show that performance variability varies per cloud operator, and use simulation experiments to show that this can affect the performance of applications, including a social online game.
In contrast, our benchmark uses real-world experiments to evaluate the effect of performance variability on \mves, which are real-time online games.


==> TECHNICAL REPORT ICPE2023 Meterstick NEW/content/7_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

%With 3~billion players world wide, and a revenue of over \$170~billion, gaming is the world's largest entertainment industry.
Online gaming is a popular and lucrative part of the entertainment industry, but raises important performance challenges.
% In this work, we focus on the performance and scalability of Minecraft and Minecraft-like games, which are important exemplars of online games in which players have fine-grained control over the virtual environment (\mves).
% Earlier work has shown that \mves scale only to 200-300\,players under favorable conditions; and to as low as 10\,players in commercial \mve{}-as-a-service operations.
%We have addressed the question 
%\emph{What limits \mve scalability?} 
In this work, we posit performance variability is an important cause for the lack of scalability
in \mves.

% %
% % \mves, a particular and highly popular type of online game,
% % in which players have fine-grained control over the virtual environment.
% %The canonical example of an \mve is Minecraft, which is currently the best selling game of all time, and has more active monthly users than there are global MacOS users.
% Next to Minecraft, hundreds of thousands of other \mve games and game modifications (mods) exist.
% % Useful to society statement?
% However, the large number of \mve players can currently only be supported by replicating isolated instances, effectively preventing players from playing together.
% Earlier work has shown that \mves scale only to 200-300 players under favorable conditions.
% However, \mves exhibit significant performance variability which can cause the number of supported players
% to drop far below the maximum.

% In this work, we posit performance variability is an important cause for the lack of scalability
% in \mves. 
We make a four-fold contribution to better understand the behavior of \mves.
\textit{First}, we propose a novel workload model for these systems, which identifies important sources of performance variability not considered elsewhere. %%%and explains it in practical \mve operation.
\textit{Second}, we design and implement \toolname, the first benchmark to evaluate performance variability in \mves.
\toolname uses realistic workload types; novel, it considers \envworkloads, and can evaluate \mves running both in self-hosted and cloud environments such as Amazon~AWS and Microsoft~Azure.
\textit{Third}, we use \toolname to perform real-world experiments and analyze the results.
We find that performance variability negatively affects players in \mves, that both \envworkloads and cloud environments can cause significant performance variability.
% and that \mves exhibit significant performance variability when using the recommended hardware configuration.
This leads us to formulate four actionable insights.
% add actionable insight: use more hardware than recommended (e.g., aws 2xlarge)
\textit{Fourth}, we release FAIR and FOSS artifacts that enable reproducibility for this work. % and open science further on.

In future work, we aim to conduct user studies to directly link our \newmetricfull~(\newmetric) values to player-perceived quality of experience.
To encourage community adoption, we aim to create a public score-board where operators of \mve{}-as-a-service can publish benchmark scores.

% developers can publish their benchmark scores for users to compare.

% to evaluate more \mves and explore a larger parameter space.
% Additionally, we aim to create a public score-board where \mve developers can publish their benchmark scores for users to compare.
% Finally, we want to conduct user studies to link values of jitter with player-perceived quality of experience for different games and \mves.

%\section*{Artifacts for Reproduction}\label{sec:artifacts}
%\todoall{Upload blinded data/tools}


==> TECHNICAL REPORT ICPE2023 Meterstick NEW/setup-comments.tex <==
%
\usepackage{xcolor}  % Colored text etc.
% \usepackage[colorinlistoftodos,prependcaption,textsize=tiny]{todonotes}
%\usepackage{xargs}                      % Use more than one optional parameter
\usepackage{mdframed}
% \usepackage{ntheorem}

% in a new commands
% Add ,disable to the options, to hide the comments
%
\definecolor{OwnAzure}{HTML}{336699}
\definecolor{OwnCerulean}{HTML}{CAE2FE}
\definecolor{OwnOliveGreen}{HTML}{556B2F}
%

\setlength{\marginparwidth}{1cm}
%\reversemarginpar

% START CODE TO MANAGE REVIEW COMMENTS AND MODIFICATIONS


\newif\ifistoreview

\istoreviewfalse

\newcommand{\setreviewson}{\istoreviewtrue}
\newcommand{\setreviewsoff}{\istoreviewfalse}

\RequirePackage{soul}
\RequirePackage{xcolor}
\RequirePackage{todonotes}

\newcommand{\alertColor}{\textcolor{red}}
\newcommand{\removeColor}{\textcolor{red}}
\newcommand{\addColor}{\textcolor{blue}}

\newcommand{\alert}[1]{\ifistoreview\alertColor{#1}\else #1\fi}
\newcommand{\remove}[1]{\ifistoreview\alertColor{#1}\else\relax\fi}
\newcommand{\add}[1]{\ifistoreview\addColor{#1}\else #1\xspace\fi}
\newcommand{\substitute}[2]{\ifistoreview\remove{#1}~\add{#2} \else #1\fi}
\newcommand{\replace}[2]{\ifistoreview\remove{#1}~\add{#2}\else #2\fi}
\newcommand{\highlight}[1]{\hl{#1}}

%\newenvironment{addtext}{\begingroup\color{blue}}{\endgroup}
\newenvironment{addtext}{\begingroup}{\endgroup}
\renewcommand{\comment}[2]{\highlight{#1}\todo[inline]{#2}}

\newcounter{info}

\newcommandx{\info}[2][1=]{\refstepcounter{info}\label{#1}\ifthenelse{\equal{#2}{}}{\todo{F\theinfo}}{\todo{F\theinfo: #2}}}
\newcommand{\refinfo}[1]{F\ref{#1}}

% From https://medium.com/@xLeitix/marking-changed-text-in-journal-revisions-8583136a4738
\theoremstyle{nonumberplain}
\newmdtheoremenv[%
  linecolor=blue,
  linewidth=2pt,
  rightline=false,
  leftline=false]{figrev}{}
% END CODE TO MANAGE REVIEW COMMENTS AND MODIFICATIONS


%
%
%
%\newcommand{\todocite}[1]{\todo[color=green!40]{#1}}
% %
% \newcommandx{\todolarge}[2][1=]{\todo[inline,size=\large,linecolor=OwnAzure,backgroundcolor=OwnCerulean,bordercolor=OwnAzure,#1]{#2}}
% %
% \newcommandx{\todoai}[2][1=]{\todo[inline,linecolor=OwnAzure,backgroundcolor=OwnCerulean,bordercolor=OwnAzure,#1]{#2}}
% % TODOs
% \newcommand{\todoall}[1]{\todo[inline, color=orange!40]{ANYONE: #1}}
% \newcommand{\todoalexandru}[1]{\todo[inline, color=orange!40]{Alexandru: #1}}
% \newcommand{\askalex}[1]{\todoalexandru{#1}}
% \newcommand{\todoalexu}[1]{\todo[inline, color=blue!40]{Alex U.: #1}}
% \newcommand{\todolaurens}[1]{\todo[inline, color=yellow!40]{Laurens: #1}}
% \newcommand{\todoerwin}[1]{\todo[inline, color=red!40]{Erwin: #1}}
% \newcommand{\todovincent}[1]{\todo[inline, color=green!40]{Vincent: #1}}
% \newcommand{\todogeorgios}[1]{\todo[inline, color=blue!40]{Georgios: #1}}
% \newcommand{\todosacheendra}[1]{\todo[inline, color=OwnAzure!40]{Sacheendra: #1}}
% \newcommand{\todotim}[1]{\todo[inline, color=OwnCerulean!20]{Tim: #1}}
% \newcommand{\todolucian}[1]{\todo[inline, color=OwnCerulean!40]{Lucian: #1}}
% \newcommand{\todoother}[1]{\todo[inline, color=cyan!40]{Other: #1}}
% \newcommand{\todojesse}[1]{\relax}%{\todo[inline, color=green!40]{Jesse: #1}}
% \newcommand{\todojd}[1]{\todojesse{#1}}

\newcommand\ab[1]{\textcolor{blue}{#1}}
\newcommand\nh[1]{\textcolor{green}{#1}}


% \newcommandx{\addref}[2][1=]
% {\todo[inline,linecolor=blue,backgroundcolor=blue!50,bordercolor=blue,#1]{Add reference. #2}}
% \newcommandx{\unsure}[2][1=]{\todo[inline, linecolor=red,backgroundcolor=red!25,bordercolor=red,#1]{#2}}
% \newcommandx{\change}[2][1=]{\todo[inline, linecolor=blue,backgroundcolor=blue!25,bordercolor=blue,#1]{#2}}
% \newcommandx{\improvement}[2][1=]{\todo[linecolor=Plum,backgroundcolor=Plum!25,bordercolor=Plum,#1]{#2}}
% \newcommandx{\thiswillnotshow}[2][1=]{\todo[disable,#1]{#2}}
%

\definecolor{darkred}{rgb}{0.5,0,0}
\definecolor{darkgreen}{rgb}{0,0.5,0}
\definecolor{darkblue}{rgb}{0,0,0.5}


%\newcommand{\todo}[1]{\noindent\textbf{\textsc{\textcolor{blue} {(TODO: #1)}}}}
% \newcommand{\note}[1]{\noindent\textbf{\textsc{\textcolor{darkgreen} {(NOTE: #1)}}}}
% \newcommand{\NOTE}[1]{\noindent\textbf{\textsc{\textcolor{red} {(IMPORTANT: #1)}}}}

\newcommand{\commentt}[3]{{\textcolor{blue}{\textbf{[#1:#2]} \{#3\} }}} % For including arbitrary comments concerning a marked text: \comment{SK}{grammar}{marked text}

==> setup-comments.tex <==
%
\usepackage{xcolor}  % Colored text etc.
% \usepackage[colorinlistoftodos,prependcaption,textsize=tiny]{todonotes}
%\usepackage{xargs}                      % Use more than one optional parameter
\usepackage{mdframed}
% \usepackage{ntheorem}

% in a new commands
% Add ,disable to the options, to hide the comments
%
\definecolor{OwnAzure}{HTML}{336699}
\definecolor{OwnCerulean}{HTML}{CAE2FE}
\definecolor{OwnOliveGreen}{HTML}{556B2F}
%

\setlength{\marginparwidth}{1cm}
%\reversemarginpar

% START CODE TO MANAGE REVIEW COMMENTS AND MODIFICATIONS


\newif\ifistoreview

\istoreviewfalse

\newcommand{\setreviewson}{\istoreviewtrue}
\newcommand{\setreviewsoff}{\istoreviewfalse}

\RequirePackage{soul}
\RequirePackage{xcolor}
\RequirePackage{todonotes}

\newcommand{\alertColor}{\textcolor{red}}
\newcommand{\removeColor}{\textcolor{red}}
\newcommand{\addColor}{\textcolor{blue}}

\newcommand{\alert}[1]{\ifistoreview\alertColor{#1}\else #1\fi}
\newcommand{\remove}[1]{\ifistoreview\alertColor{#1}\else\relax\fi}
\newcommand{\add}[1]{\ifistoreview\addColor{#1}\else #1\xspace\fi}
\newcommand{\substitute}[2]{\ifistoreview\remove{#1}~\add{#2} \else #1\fi}
\newcommand{\replace}[2]{\ifistoreview\remove{#1}~\add{#2}\else #2\fi}
\newcommand{\highlight}[1]{\hl{#1}}

%\newenvironment{addtext}{\begingroup\color{blue}}{\endgroup}
\newenvironment{addtext}{\begingroup}{\endgroup}
\renewcommand{\comment}[2]{\highlight{#1}\todo[inline]{#2}}

\newcounter{info}

\newcommandx{\info}[2][1=]{\refstepcounter{info}\label{#1}\ifthenelse{\equal{#2}{}}{\todo{F\theinfo}}{\todo{F\theinfo: #2}}}
\newcommand{\refinfo}[1]{F\ref{#1}}

% From https://medium.com/@xLeitix/marking-changed-text-in-journal-revisions-8583136a4738
\theoremstyle{nonumberplain}
\newmdtheoremenv[%
  linecolor=blue,
  linewidth=2pt,
  rightline=false,
  leftline=false]{figrev}{}
% END CODE TO MANAGE REVIEW COMMENTS AND MODIFICATIONS


%
%
%
%\newcommand{\todocite}[1]{\todo[color=green!40]{#1}}
% %
% \newcommandx{\todolarge}[2][1=]{\todo[inline,size=\large,linecolor=OwnAzure,backgroundcolor=OwnCerulean,bordercolor=OwnAzure,#1]{#2}}
% %
% \newcommandx{\todoai}[2][1=]{\todo[inline,linecolor=OwnAzure,backgroundcolor=OwnCerulean,bordercolor=OwnAzure,#1]{#2}}
% % TODOs
% \newcommand{\todoall}[1]{\todo[inline, color=orange!40]{ANYONE: #1}}
% \newcommand{\todoalexandru}[1]{\todo[inline, color=orange!40]{Alexandru: #1}}
% \newcommand{\askalex}[1]{\todoalexandru{#1}}
% \newcommand{\todoalexu}[1]{\todo[inline, color=blue!40]{Alex U.: #1}}
% \newcommand{\todolaurens}[1]{\todo[inline, color=yellow!40]{Laurens: #1}}
% \newcommand{\todoerwin}[1]{\todo[inline, color=red!40]{Erwin: #1}}
% \newcommand{\todovincent}[1]{\todo[inline, color=green!40]{Vincent: #1}}
% \newcommand{\todogeorgios}[1]{\todo[inline, color=blue!40]{Georgios: #1}}
% \newcommand{\todosacheendra}[1]{\todo[inline, color=OwnAzure!40]{Sacheendra: #1}}
% \newcommand{\todotim}[1]{\todo[inline, color=OwnCerulean!20]{Tim: #1}}
% \newcommand{\todolucian}[1]{\todo[inline, color=OwnCerulean!40]{Lucian: #1}}
% \newcommand{\todoother}[1]{\todo[inline, color=cyan!40]{Other: #1}}
% \newcommand{\todojesse}[1]{\relax}%{\todo[inline, color=green!40]{Jesse: #1}}
% \newcommand{\todojd}[1]{\todojesse{#1}}

\newcommand\ab[1]{\textcolor{blue}{#1}}
\newcommand\nh[1]{\textcolor{green}{#1}}


% \newcommandx{\addref}[2][1=]
% {\todo[inline,linecolor=blue,backgroundcolor=blue!50,bordercolor=blue,#1]{Add reference. #2}}
% \newcommandx{\unsure}[2][1=]{\todo[inline, linecolor=red,backgroundcolor=red!25,bordercolor=red,#1]{#2}}
% \newcommandx{\change}[2][1=]{\todo[inline, linecolor=blue,backgroundcolor=blue!25,bordercolor=blue,#1]{#2}}
% \newcommandx{\improvement}[2][1=]{\todo[linecolor=Plum,backgroundcolor=Plum!25,bordercolor=Plum,#1]{#2}}
% \newcommandx{\thiswillnotshow}[2][1=]{\todo[disable,#1]{#2}}
%

\definecolor{darkred}{rgb}{0.5,0,0}
\definecolor{darkgreen}{rgb}{0,0.5,0}
\definecolor{darkblue}{rgb}{0,0,0.5}


%\newcommand{\todo}[1]{\noindent\textbf{\textsc{\textcolor{blue} {(TODO: #1)}}}}
% \newcommand{\note}[1]{\noindent\textbf{\textsc{\textcolor{darkgreen} {(NOTE: #1)}}}}
% \newcommand{\NOTE}[1]{\noindent\textbf{\textsc{\textcolor{red} {(IMPORTANT: #1)}}}}

\newcommand{\commentt}[3]{{\textcolor{blue}{\textbf{[#1:#2]} \{#3\} }}} % For including arbitrary comments concerning a marked text: \comment{SK}{grammar}{marked text}
